"I Want It That Way": Enabling Interactive Decision Support Using Large Language Models and Constraint Programming

A critical factor in the success of decision support systems is the accurate modeling of user preferences. Psychology research has demonstrated that users often develop their preferences during the elicitation process, highlighting the pivotal role of system-user interaction in developing personalized systems. This paper introduces a novel approach, combining Large Language Models (LLMs) with Constraint Programming to facilitate interactive decision support. We study this hybrid framework through the lens of meeting scheduling, a time-consuming daily activity faced by a multitude of information workers. We conduct three studies to evaluate the novel framework, including a diary study (n=64) to characterize contextual scheduling preferences, a quantitative evaluation of the system's performance, and a user study (n=10) with a prototype system. Our work highlights the potential for a hybrid LLM and optimization approach for iterative preference elicitation and design considerations for building systems that support human-system collaborative decision-making processes.

==> Misc/CSCW_Background.tex <==
\section{Background}
Successful time management is a key aspect of human well-being and is crucial for our biological~\cite{healy2008breaks}, cognitive~\cite{schmidt2007time}, and social~\cite{romero2017influence, bodker2013calendars} functions.
Organizationally, effective scheduling is even more salient for increasingly complex and globalized businesses, whose employees must navigate myriad factors to arrange time in their calendars for meeting and collaborating~\cite{cao2021large,mok2023challenging,hongladarom2002web}.
Without finding time for meetings, workers would be disafforded an immediate way of exchanging information~\cite{mell2021bridging,mok2023challenging} that would allow collaborators to converge on common ground~\cite{dennis1999rethinking} and reduce delays in coordination~\cite{olson2000distance, espinosa2011time}.
% The intricacies of workplace scheduling has therefore led to many endeavors to design scheduling systems that capture different temporal needs~\cite{tullio2002augmenting,chen2012spalendar,kim2018learning,cranshaw2017calendar}.
Indeed, the intricacies of workplace scheduling have been further complicated by shifts towards remote work induced by COVID-19~\cite{teevan2022microsoft, yang2022effects}, blurring the boundary between work and personal life~\cite{allen2021boundary,hakkila2020practical}.

Our study clarifies the complex preferences and behaviors underpinning how information workers schedule, and is situated against two bodies of related research delineated in this section.
First, we survey the literature on \textit{work rhythms} and the temporal patterns according to which people undertake personal and labor tasks.
Second, we examine research that aim to design calendaring systems by capturing anecdotal and theoretical accounts of workers' temporal preferences.  

% \lm{We should introduce why we're studying meetings in the first place}

% \lm{TODO move this }
% % Individual workers have difficulties with scheduling - balance individual time and productivity.
% In the face of this complexity, meeting scheduling offers a mechanism to concretely shape working structures in a way that aligns needs and preferences of individuals that can optimize for both collaboration and individual productivity~\cite{kaur2020optimizing}.
% % However, in order to design a scheduling a system that potentially align with user preferences, a system must model and understand users diverse preferences and needs~.
% Evidence suggests that this is particularly challenging in hybrid and remote contexts. 
% While employees cite focus time, increased collaboration, and productivity as reasons to increase their time in the office, the same workers also cite many of the same reasons as motivation for increasing their time working from home \cite{teevan2022microsoft}. 
% This so-called hybrid paradox, describes how individuals balance the need to do focused individual work with the need to collaborate with others, while navigating work-life boundaries.
% % To optimize schedules, information workers need to be aware of work rhythms, capture daily preferences, and identify the discrepancies between constraints and preferences to concretely shape their workday~\cite{berry2007balancing, oh2005calendar}.

% \lm{TODO move this} Successful time management is a key aspect of human well-being and is crucial for our biological~\cite{healy2008breaks}, cognitive~\cite{schmidt2007time}, and social~\cite{romero2017influence, bodker2013calendars} functions.
% Organizationally, effective scheduling is even more salient for increasingly complex and globalized businesses, whose employees must navigate myriad factors to arrange time in their calendars for meeting and collaborating~\cite{cao2021large,mok2023challenging,hongladarom2002web}.
% Without finding time for meetings, workers would be disafforded an immediate way of exchanging information~\cite{mell2021bridging,mok2023challenging} that would allow collaborators to converge on common ground~\cite{dennis1999rethinking} and reduce delays in coordination~\cite{olson2000distance, espinosa2011time}.
% The intricacies of workplace scheduling has therefore led to many endeavors to design scheduling systems that capture different temporal needs~\cite{tullio2002augmenting,chen2012spalendar,kim2018learning,cranshaw2017calendar}.

% % Information workers are often faced with the challenge of balancing the need to do focused individual work with the need to collaborate with others. While individual work is important for completing tasks, collaborating with others is also essential for achieving goals, solving problems, and fostering creativity. However, as the boundaries between work and life are becoming increasingly blurred, information workers must navigate this balance while also maintaining a healthy work-life boundary. This can be accomplished by setting realistic expectations and goals, creating clear boundaries between work and personal time, and utilizing tools and technologies that allow for seamless collaboration while also supporting focus and productivity.

% % move this to bg
% Despite these challenges, synchronous collaboration via meetings stays necessary for valuable immediacy of information change between teams~\cite{mell2021bridging,mok2023challenging}. 
% Media synchronicity theory, for instance, argues that asynchronous communication is not sufficient; synchronous communications are needed for convergence upon a shared understanding of information~\cite{dennis2008media,dennis1999rethinking}. 
% This theory is supported by a wide range of empirical evidence, including the finding that synchronous communication facilitates rapid feedback and reduce delays in coordination~\cite{olson2000distance,tang2011your,cummings2009crossing,morrison2020challenges,agerfalk2005framework,espinosa2006effect,espinosa2011time}. 
% % Without synchronicity, teams must wait for information and expertise from collaborators~\cite{agerfalk2005framework,morrison2020challenges,cummings2011geography},
% % particularly for cross time zone teams. This asynchronous delay can produce siloed and static collaboration patterns~\cite{yang2022effects,ahuja1999network,ahuja2003individual,suh2011influence}.
% In total, the boundaries between work and personal life have become more blurred for many workers~\cite{allen2021boundary,hakkila2020practical}

% % \shs{I tried to adapt this paragraph, but I am struggling to clearly draw the connection here.} \bs{Same! Like the first sentence, but not the second.} \lm{The gap for me is more between P2 and P3 rather than P3 and P4.} \ls{still feel the p2 and p3 is not connected well }

\subsection{The rhythm of work}
Information workers exhibit rhythm in their daily life, including when they usually start the day, attend meetings and take lunch breaks~\cite{reddy2002finger,jackson2011collaborative,breideband2022home}. 
These rhythms play a vital role in workdays by helping to maintain working productivity and balance work and personal life~\cite{tang2001connexus,begole2002work,begole2003rhythm,mark2014bored}. 
Here, we examine key aspects of these rhythms that can influence work patterns and organizational outcomes. 
%day of week
Firstly, a rich body of CSCW work has explored rhythms of work related to the \textbf{day of week} in different contexts, including doctors, developers, scientific researchers, and information workers~\cite{begole2002work,reddy2002finger,begole2003rhythm,jackson2011collaborative,mark2014bored,meyer2019today,breideband2022home}. 
Previous research found that some developers organize their day of the week based on the activities they usually conduct, such as bug-fixing day, meeting day, or planning day~\cite{meyer2019today}. 
Developers reported that they usually scheduled ``no meeting days'' where they reserve one weekday, such as Monday, to focus on coding and development. 
Researchers proposed a hypothesis on the ``Blue Monday effect'', where people are in bad mood on Mondays, which affects the ability to focus on work~\cite{stone1985prospective}. 
Faced with this hypothesis, a previous in-situ tracking study with information workers found that people report Monday being the most bored, but at the same time also the most focused~\cite{mark2014bored}. 

%chronotype
Research has also found that \textbf{circadian rhythms} and people's inner clock have strong influences on people's daily activities, including sleep, work productivity, and mood~\cite{cajochen2003role,murray2010circadian,steinhardt2014reconciling,jun2019circadian,janbocke2020finding,raiha2021evening,breideband2022home}. 
Previous research used chronotypes to describe individuals' circadian preferences, such as ``early birds'' or ``night owls''~\cite{jun2019circadian,schmidt2007time}. 
Morning chronotypes often awaken, prefer to start working, and feel tired earlier in the day. Others are ``night owls'' who experience the patterns later in the day and tend to awaken later, stay up working, and go to bed later. 
Growing evidence showed that circadian rhythms impact individual cognition and productivity as well as group collaborative work~\cite{jun2019circadian,wieth2011time,folkard2003shift,schmidt2007time}. 
Researchers even developed calendar applications that incorporate chronotype information to help people manage their day~\cite{janbocke2020finding}. 

% hybrid and preferred working hours
The modality of work also influences work rhythms. 
For instance, \textbf{remote or hybrid workers} with families play multiple social roles in life \cite{grimes2008life}. 
They need to not only manage schedules with teams but also coordinate with other family members on responsibilities, such as picking up children from daycare. 
Previous CSCW work investigated the usage of calendars with family and found that individuals used calendars to build shared understanding and reduce tensions~\cite{elliot2005awareness,hakkila2020practical,neustaedter2009calendar,bodker2013calendars}. 
Remote modalities are also determined by whether co-workers are \textbf{geographically disperse}, which makes it more difficult for collaborators to capture and maintain rhythmic patterns~\cite{olson2000distance}. 
% For example, meeting conflicts and cross-time zone meeting schedules become barriers to smooth team collaboration~\cite{MSTriplePeak}.
In turn, lack of awareness of rhythms in a distributed team increases the cost of coordinating meetings and collaborations~\cite{begole2003rhythm,jackson2011collaborative,morrison2020challenges}.
When teams are also \textbf{temporally distanced} across different timezones, meetings become significantly harder to schedule but more important for keeping collaborations diverse and well-connected~\cite{mok2023challenging}.
% \ls{cite some findings from Lillio's paper}

% 'VID
These considerations have become even more salient during the \textbf{COVID-19 pandemic}, during which companies have shifted towards infrastructure and business models that enable employees to work remotely and from home~\cite{defilippis2020collaborating,yang2022effects}. 
Studies have shown that workdays have become longer~\cite{MSWTI} and blurred with personal life~\cite{allen2021boundary,hakkila2020practical}. 
% Workers have recently shifted towards remote or hybrid working modalities~\cite{yang2022effects}. 
A previous study on workers found that the 9-to-5 workday is fading in an age of remote and hybrid work and some people have grown accustomed to the ``triple peak day'', where there is a third peak raised after 9-to-5 workday hours~\cite{MSTriplePeak}. 
It raised the question that whether workers perceive this triple peak as more flexible or as an encroachment on personal hours that are normally used for family time or social life. 
Simultaneously, there are also signs that teams may have become less productive~\cite{gibbs2021work}, less focused~\cite{cao2021large}, and less connected~\cite{yang2022effects}. 

% productivity 
The rhythms are therefore viewed as important factors in helping balance \textbf{productivity and well-being}. 
Workers often block time on their calendars to reduce distractions and prevent interruptions \cite{mark2018effects}. 
An interruption at the wrong time, e.g. when users are in a state of flow, can result in lower task productivity and increased frustration~\cite{mihaly1997finding,mark2008cost,mcternan2013depression}. However, long continuous working hours  without breaks can induce more mental stress, so people always take breaks due to tiredness and boredom \cite{epstein2016taking,strongman2000taking}. Previous research showed that work breaks, such as stepping away from one’s work area to get food or drink, can contribute positively to workers' mental and physical well-being and improve their creativity and productivity~\cite{healy2008breaks,epstein2016taking,cambo2017breaksense,mark2018effects,kaur2020optimizing}. 


\subsection{Capturing scheduling preferences}\label{section:bg:calendar}
% \shs{Bahar has a really great doc on this, Lu, that you may be able to adapt content from.}
% \ls{adapting some content from Bahar's document to here}

% Meeting scheduling is a well-known naturally distributed agreement problem \cite{crawford2009learning,benhassine2007agent}. It is a routine, tedious, and time-consuming daily activity, which requires coordination and cooperation among all attendees. The main challenge is how to find an agreed time among various constraints, such as participant’s schedules, preferences or priorities \cite{ephrati1994meet}.

It is therefore unsurprising, given the complex temporal dynamics governing people's workday, that scheduling is a complex personal behavior. 
Whether the user is initiating a new meeting or responding to a meeting request she chooses an action with multiple objectives in mind~\cite{berry2007balancing,oh2005calendar}. 
For instance, when trying to schedule a new meeting, the user may want to minimize change to her existing meetings, and she takes a scheduling action that best compromises the overall objectives, such as: minimizing travel time, maximizing a contiguous meeting time, choosing a preferred meeting location, etc. 
As a result, a calendar scheduling system that tries to predict the best scheduling actions needs to know user's preferences and priorities \cite{oh2005calendar}.

% Preference learning provides the means for modeling and predicting people’s desires and this makes it a crucial aspect in modern applications such as decision support systems \cite{chajewska2000making}, recommender systems (Blythe 2002; Blei et al. 2003), and personalized devices (Clyde et al. 1993; Heskes and de Vries 2005).

Learning and incorporating personal preference in calendar scheduling systems received previous attention~\cite{dent1992personal,mitchell1994experience,sen1997satisfying,chajewska2000making,tullio2002augmenting,oh2005calendar,gervasio2005active,brzozowski2006grouptime,krzywicki2010adaptive,kim2018learning}. 
\citeauthor{mitchell1994experience} proposed Calendar Apprentice (CAP) which is a decision tree based calendar manager that can learn decision rules for predicting the values of schedule attributes such as day, time and location~\cite{mitchell1994experience}. 
PLIANT used an active learning approach where the learning system can learn user preferences from the feedback that naturally occurs during interactive scheduling \cite{gervasio2005active}. 

To understand personal preferences, scheduling systems must deal with challenges in  preference elicitation.
The user may not be fully aware of their preferences or be able to express them~\cite{berry2007balancing}. 
Even in cases where the user does know about their preferences and is able to express them, she may not be willing to input them into the system, especially if the elicitation process is burdensome. 
The first approach to the elicitation of general scheduling preferences aims to derive rankings of schedule options by showing user-specific examples as part of an elicitation phase. 
GroupTime~\cite{brzozowski2006grouptime} is a scheduling system that takes such an example-driven approach. 
\citeauthor{viappiani2006evaluating} show that presenting users with carefully chosen examples can help stimulate their preferences, a technique known as example critiquing~\cite{viappiani2006evaluating}. 
An alternative approach to elicitation requires the user to enter the parameters of the preference model directly. 
The scheduling system of \citeauthor{haynes1997automated} takes such a model-driven approach. The advantage of this approach is that the elicitation period can be shorter because the information elicited has greater entropy \cite{haynes1997automated}. 
The significant disadvantage is that users must comprehend the model, rather than examples that are possibly easier to comprehend.

Some scheduling systems took the user-centered approach to understand and elicit user preferences. 
In PTIME \cite{berry2007balancing}, they first conduct a structured interview  with subjects to capture their criteria on scheduling and used the findings of the user study as well as features suggested in prior work in the literature (e.g., \cite{kozierok1993learning,mitchell1994experience,brzozowski2006grouptime}), to identify seven criteria consistent across different users, such as duration of meetings and scheduling windows for the requested meetings.
Later, the system provided an interactive visual interface that present several statements around scheduling criteria such as ``avoid rescheduling'' or ``meeting duration'' and ask participants to rank the importance of each criterion. 
However, this system provided general criteria for the meeting within the days and there are still a large number of preference categories, such as ``meeting gaps'', that are not captured. 

\xhdr{Relation to this work}
Together, this rich body of research paints a nuanced picture of how an individual's workday can be influenced by various temporal preferences and necessities, and how these preferences can be distilled into guidance for designing scheduling aids.
However, several gaps remain in our understanding of these calendaring dynamics, which we address at present.

Firstly, while the literature identifies several situation-specific preferences (e.g. Mondays~\cite{stone1985prospective,mark2014bored} and no-meeting days~\cite{meyer2019today}), we still lack a generalized taxonomy of temporal needs capturing different time scales and temporal relationships like breaks.
Furthermore, the relationship between self-reported, stated calendaring preferences and what workers do in practice remains unclear.
Although employees in large organizations may not easily meet their scheduling preferences, it is unknown whether their actual calendars are populated with sub-optimal timeslots~--~nor, indeed, what their actual calendars look like in general.
Finally, the major workplace changes induced by COVID-19 cast much uncertainty over established observations of scheduling behaviors. 
On the one hand, increasingly flexible workdays may allow calendaring at preferable hours; on the other, the blending of work and non-work days may impinge upon times reserved for offline obligations.

Our work thus contributes a mixed-methods contextual inquiry and survey to disentangle scheduling preferences, complimented by a large-scale characterization of workers' \textit{in situ} calendaring behaviors.
This endeavors to fill the empirical gaps in our understanding of how calendars can be better organized, and is the first to do so across the entirety of a multinational organization in the post-pandemic paradigm of work. 

% Despite previous systems eliciting preference categories in scheduling, we still lack a holistic understanding of the categories of scheduling preference. 
% To this end, our study aims to provide a holistic category of information workers' preferences. 
% Our study further compared the current practice and workers' preferences to find the misalignment. 


% \lm{move to end} In our study, we aim to investigate the typical day-of-week rhythms that information workers more broadly exhibited, with a focus on meeting times, and try to understand the variation in these rhythms. 
% % \ls{try to distinguish our work from previous work here, we used mixed method study?}
% \lm{move this}In our survey, we further investigated how family responsibilities influence patterns in a worker's daily life and how workers manage this.
% \lm{move}We try to reveal insights into workers' preferred working hours including their challenges and perceptions of the current working schedule.
% \lm{move this} Our work, which seeks to understand the practice and rhythms of information workers' workdays in the post-pandemic era, therefore, is crucial for both individual workers and organizational teams. 
% \lm{move to end} We seek to explore how workers take breaks on their meeting schedule such that they can maintain productivity and happiness. 


% These studies illustrate the broad spectrum of characteristics exhibited by the rhythm of work and its relationship to key organizational outcomes. 
% However, 


% \lm{The background is very comprehensive; there's a lot of room here to tie everything together and situate our contributions more clearly against the lit. This should help focus our narrative for reviewers who are concerned about obviousness. }\bs{Agreed! I can see at least two distinctions to highlight for reinforcing our contributions: (a) revisiting this research post pandemic and in light of more flexible and diverse workdays; (b) Studying stated preferences alongside observed practices at scale and looking at the alignment between the two.}

==> deprecated/Intro-WIP.tex <==
\section{Introduction}
\bs{Note to all: (1) this is mainly a WIP Intro. I'm working on the version I'm adding here outside this overleaf. You can ignore this for now. (2) I'm working on Intro and RW concurrently as the new framing requires a lot of reading and including new literature that weren't previously explored.}
Knowing what a user likes and dislikes, i.e., their preferences, is important for intelligent systems in many domains. Users preferences and constraints are particularly crucial for the success of systems that provide decision or negotiation support. 
Decision support systems, while share many similarities with Recommender Systems,  focus more on the decision process itself. This includes helping the user to discover and enter their preferences, understand the link between preferences and decision outcomes and analyzing the steps taken in the process.

\js{We are using intelligent system, recommender system, and decision support sytem. Intended?}

Eliciting preference information from a user is challenging. On one hand, the user may not be fully aware of their preferences or be able to express it (at least via the elicitation mechanism offered) [7]. On the other hand, even in cases where the user does know about their preferences and is able to express them, she may not be willing to input them to the system, especially if the elicitation process is burdensome. Moreover, the very process of elicitation itself is known to reshape — and at worst bias — the information provided; preferences can even be created by the elicitation process [13, 14]. 

Psychology research has shown that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions (Slovic, 1995; for a comprehensive review, see Lichtenstein \& Slovic, 2006). 
There is a body of literature that suggests people often do not have well-defined preferences. Instead they construct them during the elicitation process. Put differently, preferences are invented rather than found (Johnson, Steffel, \& Goldstein, 2005), more like the product of architecture than of archaeology (Gregory, Lichtenstein, \& Slovic, 1993; Payne, Bettman, \& Schkade, 1999). This implies that the interaction between the system and a user can greatly influence the quality of the preference information and the user’s acceptance of the results provided by the system. 

Past research has also attributed these findings to the inherent limitations of individuals memory, attention and knowledge. Preference elicitation tools and techniques [Rs] are known to assist the human decision maker in overcoming these limitations. These computational aids can assist humans in identifying good quality solutions by interactively learning their preferences, which are unobserved, and using them to suggest progressively better recommendations until a satisfactory one is found.

\bs{Transition to meeting scheduling as our use case and justifying the characteristics of meeting scheduling that makes it a suitable scenario to explore preference elicitation for]} We focus our work on meeting scheduling as an instance of a complex spatial-temporal decision making process that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. For instance, ...

\bs{[Placeholder for limitations of existing approaches]} Existing interfaces aiming at eliciting preferences from users range from systems that explicitly ask their users to fill in a long list of values for all the attributes of a certain item to systems that implicitly learn preferences from the user’s ratings or past behavior and comparison to other users of the system [R]. Both extremes are not likely to be successful if we want the user to stay engaged with the system and trust the system’s advice. First of all it is not sensible to ask a large number of elicitation questions that are cognitively demanding to the user. Using implicit techniques to get a preference model on the other hand bears the danger that the elicited model is not accurate [R]. This might lead to the problem that the users cannot comprehend the advice from the system.

\bs{Transition to design implications of past research that guided our design choices for this hybrid LLM-CP approach.}



==> deprecated/intro_sep14_828pm.tex <==
\section{Introduction}
% Knowing what a user likes and dislikes, i.e., their preferences, is important for intelligent systems in many domains. Users' preferences and constraints are particularly crucial for the success of systems that provide decision or negotiation support. 
Understanding what a user likes and dislikes, i.e., their preferences, is crucial for the success of intelligent systems that provide decision and negotiation support across many domains.
% Decision support systems, while sharing many similarities with Recommender Systems,  focus more on the decision process itself. This includes helping the user to discover and enter their preferences, understand the link between preferences and decision outcomes and analyzing the steps taken in the process.
Decision support systems target the decision-making process itself, helping the user: discover and articulate their preferences, understand the link between preferences and decision outcomes, and analyze the steps taken in the process.
However, eliciting preference information from a user to inform such a decision process is challenging. This challenge manifests not only as a limitation of the algorithms for elicitating or representing preferences but also as an inherent difficulty of users knowing about or expressing their desired solutions. 

Prior psychology research~\cite{lichtenstein2006construction,Slovic1995construction} has shown that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions which can be attributed to the inherent limitations of individuals' memory, attention, and knowledge. 
%In many situations, individuals do not really know what they prefer.
While a variety of preferences are carried in memory, specific preferences are constructed as the situation arises~\cite{payne1992behavioral,payne1993adaptive}, and more concretely, when (1) some decision elements may be unfamiliar to the individual; (2) the available choices may present a conflict among known preferences (i.e., trade-offs are needed); and (3) it is difficult to translate positive and negative feelings into a numerical response, even when the preferences are clear.
In these situations, the space of possible outcomes may be too large to explicitly enumerate, and the solution must be synthesized via constrained optimization. 
These challenges are shared across widespread decision-making scenarios, such as meeting scheduling, travel planning or purchasing a house.

Preference elicitation tools and techniques \cite{goldsmith2008preference} are known to assist human decision-makers in overcoming some of their inherent memory or knowledge limitations. However, the constructive nature of human preferences implies that the interaction between the system and a user can greatly influence the quality of the preference information \cite{chen2009interaction, pommeranz2012designing, johnson2005making} and the user's acceptance of the results provided by the system \cite{carenini2002constructed}.
Essentially, a preference elicitation interface needs to extract information from the user's mental representation of that preference and translate it into a representation the system can reason within an iterative, non-linear process.% Yet, this translation process entails an iterative loop and is not a linear, one-way process. 
% \bs{Add(?): In this work we are exploring the design of an effective preference elicitation interface that is aligned with how humans preferences develop throughout the decision making process ...}
% In this paper, we focus on the design of an interactive preference elicitation interface which connects the two sides of this loop. 

Our approach draws on established research \cite{payne1993adaptive, payne1992behavioral, simon2004construction}  to design effective elicitation mechanisms that actively support user decision-making. 
First, decades of HCI research highlight the importance of a collaborative environment wherein both the user and the system can seamlessly exchange information and jointly tackle decision-making challenges ~\cite{peintner2008preferences}. 
Second, studies in supporting preference construction suggest that the system should contextualize the decision-making process \cite{payne1993adaptive, Slovic1995construction, pu2003user} provide concrete examples for users to critique \cite{pu2003user, chen2012critiquing, mcginty2010evolution}, along with immediate feedback to help users grasp the correlation between their stated preferences and system suggestions \cite{carenini2002constructed}. 
Finally, the preference incorporation algorithm needs to elicit user preferences incrementally \cite{pu2003user} to account for evolving preferences \cite{pommeranz2012designing, ardissono2003framework}. %Additionally, in multi-attribute decision theory (MAUT~\cite{edwards1992multiattribute,keeney1993decisions, hammond2015smart}), preferences are represented as utility functions or embedded as constraints, leading to the application of constraint satisfaction techniques for managing trade-offs ~\cite{simon2004construction}.
%heory have also pointed out the advantage of eliciting user preferences incrementally \cite{pu2003user}. Continuous updates of the preference model and adaptations of the interface support the constructive nature of human preferences as they may evolve during the interaction with the system \cite{pommeranz2012designing, ardissono2003framework}.
% Existing literature on adaptive decision-making theory \cite{payne1993adaptive}, preference construction \cite{payne1992behavioral}, and decision-making by constraint satisfaction \cite{simon2004construction} provide guidelines for effective elicitation mechanisms that actively support users. 
%First, because the preference construction process is highly influenced by the decision context and handling of the preference elicitation, it is important for the elicitation mechanism to show the decision context and consequences of decisions. 
%The decision context can also provide specific examples for users to critique and refine their preferences as well as immediate feedback that allows users to better understand the link between their stated preferences and suggestions provided by the system.
%Second, decades of HCI research highlight the importance of the collaboration between the system and user in designing effective and personalized decision support systems. In this collaboration, users' ability to interpret system information influences their ability to express preferences and reach successful decisions~\cite{peintner2008preferences}.
%An ideal system leverages natural, flexible, and intuitive interactions to facilitate preference elicitation and communicate its suggestions.
% This collaborative system should enable users to seamlessly participate in the preference elicitation and decision-making process through natural and flexible interaction mechanisms. Simultaneously, it should incorporate transparent mechanisms for the system to communicate its suggestions.\\
%This collaborative system needs to allow for natural and flexible interaction mechanisms for the user to be seamlessly involved in the process of preference elicitation and decision making on one hand, and transparent mechanisms for the system to communicate system suggestions, on the other.
% Finally, previous research \cite{simon2004construction} investigated preference construction within the paradigm of multi-attribute decision theory (MAUT; see e.g., \cite{edwards1992multiattribute}; Hammond, Keeney, \& Raiffa, 1999). In fact, the majority of decision support systems are based on multi-attribute utility theory (MAUT) \cite{keeney1993decisions} and, therefore, represent preferences in form of utility functions [R]. 
%Finally, preference construction within the paradigm of multi-attribute decision theory (MAUT~\cite{edwards1992multiattribute,keeney1993decisions, hammond2015smart}) represents preferences as utility functions or embeds them as constraints \cite{simon2004construction} [R].
% As a result, constraint satisfaction techniques have been used to automate the process of decision making in various scenarios, as it is aligned with how humans make decisions in complex scenarios and especially when trafe-offs are needed \cite{simon2004construction}. 
%As a result, constraint satisfaction techniques have been used to automate the decision-making process in complex scenarios where humans consider trade-offs~\cite{simon2004construction}. 
% \bs{This last guideline needs to be simplified to clarify the main point: Preference construction as constraint satisfaction is the right approach to take as this is how humans do it, and that's what we did.}

However even once preferences are elicited, finding a solution that best meets them represents a challenging decision making task. Optimization models such as Constraint Programming (CP)  are a natural fit for solving this complex reasoning problem and have been successfully applied in a range of complex decision problems. CP specifically aligns with multi-attribute decision theory \cite{edwards1992multiattribute,keeney1993decisions, hammond2015smart} where preferences are represented as utility functions or embedded as constraints, and constraint satisfaction techniques for leveraged to manage trade-offs ~\cite{simon2004construction}. However, traditional optimization approaches require full knowledge of the model's specification---including a fully specified objective and all relevant constraints. This is at odds with how users approach complex and contextual decision-making tasks where they often do not know relevant preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most users. 
Finally, these optimization approaches must function as dynamic and incremental reasoning engines: users actively construct and adjust their preferences while the system continuously learns and embeds their preferences, offering increasingly improved suggestions until a satisfactory one is achieved. 
% \bs{Shift to introducing our framework.}

% In this paper, we explore an innovative framework that integrates Large Language Models (LLMs) with optimization models. This combination leverages the versatility of LLMs as powerful multi-purpose tools, offering adaptable interactivity and advanced language understanding across various human-in-the-loop applications. \bs{A placeholder for now ...}
In this paper, we explore an innovative framework that supports  iterative preference elicitation, aligning with how humans develop or construct preferences in their decision-making. Elicited preferences are embedded into specific constraints that can be solved within an optimization setting.
We leverage (1) Large Language Models (LLMs) to facilitate natural and intuitive communication of preferences and suggestions as well as to reason about how preferences should be incorporated and translated into structured constraint functions and (2) CP techniques to reason over the space of outcomes and find optimal solutions given incorporated constraints. 
% \bs{Add(?): In this work we are exploring the design of an effective preference elicitation interface that is aligned with how humans preferences develop throughout the decision making process ...}
%\bs{Thinking of mentioning meeting scheduling as our scenario or use case for evaluating along with other aspects of the evaluation including the diary study and final user study.}
We evaluate this framework for interactive decision support systems through the lens of meeting scheduling---a routine, tedious, and time-consuming daily activity faced by a multitude of information workers. 
At its core, scheduling a meeting is a complex spatial-temporal task that is highly contextual, and finding a suitable meeting time may require reasoning over conflicting preferences, constraints, and priorities \cite{baharcscw}.
It is also an incremental and continuous process that requires iteratively refining candidate solutions in a more or less greedy fashion \cite{brzozowski2006grouptime}. 
Therefore, interactive decision support tools are a natural fit for scheduling as they can provide contextualized and interactive support for the complex reasoning that is necessary to complete the task. 

We introduce \system, a hybrid LLM and CP approach that capitalizes on the benefits of both technologies to build an interactive decision support system for meeting scheduling. 
\system~ is designed to facilitate human-system collaboration that encompasses two key components: Preference Construction and Preference Incorporation. \textit{Preference Construction} is the process by which users of the system \textit{evaluate} candidate decisions (i.e., suggested meeting times) and \textit{express} new preferences and constraints that need to be integrated into the system. \textit{Preference Incorporation} is a mirror of the construction process from the system perspective and involves \textit{embedding} expressed user preferences in a form that can be used by the system to \textit{generate} new suggested decisions. We refer to the entire process of iteratively eliciting preferences via generating and critiquing suggestions as \textit{Preference Elicitation}. 
Because preference elicitation is an iterative process, \system~ unifies Preference Construction and Preference Incorporation into one dynamic loop where preferences are elicited in conjunction with refined suggestion generations. Figure \ref{fig:interaction_loop} outlines the key components of our interactive decision support system for meeting scheduling. 

%We decompose the problem into two primary components: Preference Construction, and Preference Incorporation. 
%Preference elicitation is the broader task of eliciting user preferences in response to decision suggestions, specifically suggested meeting times. It encompases three key phases: (A) Evaluation of suggested times, (B) Internal construction of a new preference in response to the time, and (C) the externalizing of that preference the system. Once a new preference has been articualted, the goal of the second component \textit{Preference Incorporation} is to integrate the preference to present a refined suggestion. 

We conducted three studies to better understand preference elicitation in the context of meeting scheduling.
First, we study how preferences are constructed via a diary study that collected naturalistic preferences in the moment of scheduling (n=64, Section \ref{sec:diary}). 
Informed by the results of the diary study, we then introduce \system~(Section \ref{sec:architecture}) and quantitatively evaluate the system's capabilities for preference incorporation (Section \ref{sec:quant_eval}).
Finally, we conduct a user study (n=10, Section \ref{sec:user_study}) with a prototype system to observe the iterative preference elicitation flow in situ and to inform future design improvements for interactive decision support systems.
%hrough our study, we confirm that participants' preferences are constructed in the iterative preference elicitation process in response to suggestions that were generated by the system that incorporated their preferences. 
Through our study, we confirm that participants' preferences are indeed constructed through the iterative preference elicitation process of evaluating dynamic time suggestions that incorporate their feedback.
We also identify that system explanations play a huge role in bridging the gap between understanding the system and expressing preferences, and contrasted suggestions not only give users a sense of agency but also help make the decision-making process efficient.
Our work highlights the potential for a hybrid LLM and optimization approach for iterative preference elicitation and design considerations for building systems that support human-system collaborative decision-making processes.

%Loop description
 \begin{figure}[!t]
     \centering
      \includegraphics[width=\textwidth]{figures/interaction_loop.png}
         \vspace{-0.4cm}
           \caption{An overview of the interactive loop for conversational decision support. The loop is initiated via an initial time suggestion (or set of suggestions) by the system presented to the user (A). During \textit{Preference Construction} users evaluate a proposed suggestion (C) and either express a new preference (D) to improve the given suggestion, or accept the current suggestion. New preferences are integrated into the system during \textit{Preference Incorporation} which requires the system to both embed the stated preference into the system (W) and then use it to generate a new time suggestion (F). This process is iterated until a suitable time is found.
           }
\label{fig:interaction_loop}
\end{figure}


==> deprecated/introduction-before-merge.tex <==
\section{Introduction}
% Knowing what a user likes and dislikes, i.e., their preferences, is important for intelligent systems in many domains. Users' preferences and constraints are particularly crucial for the success of systems that provide decision or negotiation support. 
Understanding what a user likes and dislikes, i.e., their preferences, is crucial for the success of intelligent systems that provide decision and negotiation support across many domains.
% Decision support systems, while sharing many similarities with Recommender Systems,  focus more on the decision process itself. This includes helping the user to discover and enter their preferences, understand the link between preferences and decision outcomes and analyzing the steps taken in the process.
Decision support systems target the decision-making process itself, helping the user: discover and articulate their preferences, understand the link between preferences and decision outcomes, and analyze the steps taken in the process.
However, eliciting preference information from a user to inform such a decision process is challenging. This challenge manifests not only as a limitation of the algorithms for elicitating or representing preferences but also as an inherent difficulty of users knowing about or expressing their desired solutions. 

Prior psychology research~\cite{lichtenstein2006construction,Slovic1995construction} has shown that individuals are often: unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions, attributing to the inherent limitations of individuals' memory, attention, and knowledge. 
In many situations, individuals do not really know what they prefer.
While a variety of preferences are carried in memory, specific preferences are constructed as the situation arises~\cite{payne1992behavioral,payne1993adaptive} when (1) some decision elements may be unfamiliar to the individual; (2) the available choices may present a conflict among known preferences (i.e., trade-offs are needed); and (3) it is difficult to translate positive and negative feelings into a numerical response, even when the preferences are clear.
In these situations, the space of possible outcomes is too large to explicitly enumerate, and the solution must be synthesized via constrained optimization. 
These challenges are shared across widespread decision-making scenarios, such as meeting scheduling, purchasing, or resource allocation.

Preference elicitation tools and techniques \cite{goldsmith2008preference} are known to assist the human decision-maker in overcoming some of their inherent memory or knowledge limitations. However, the constructive nature of human preferences implies that the interaction between the system and a user can greatly influence the quality of the preference information [R] and the user's acceptance of the results provided by the system \cite{carenini2002constructed}.
Essentially, a preference elicitation interface needs to extract information from the user's mental representation of that preference and translate it into a representation the system can reason within an iterative, non-linear process.% Yet, this translation process entails an iterative loop and is not a linear, one-way process. 
% \bs{Add(?): In this work we are exploring the design of an effective preference elicitation interface that is aligned with how humans preferences develop throughout the decision making process ...}
% In this paper, we focus on the design of an interactive preference elicitation interface which connects the two sides of this loop. 


Here, existing literature on adaptive decision-making theory [R], preference construction [R], and decision-making by constraint satisfaction [R] provides guidelines for effective elicitation mechanisms that actively support the users. 
First, because the preference construction process is highly influenced by the decision context and the handling of the preference elicitation, it is important for the elicitation mechanism to show the decision context and the consequences of decisions. 
This decision context can also provide specific examples to be critiqued by the users to refine their preferences as well as immediate feedback that allows the users to better understand the link between their stated preferences and the suggestions provided by the system.
Second, decades of HCI research highlight the importance of the collaboration between the system and the user in designing effective and personalized decision support systems. In this collaboration, the users' ability to interpret system information influences their ability to express preferences and reach successful decisions~\cite{peintner2008preferences}.
An ideal system leverages natural, flexible, and intuitive interactions to facilitate preference elicitation and communicate its suggestions.
% This collaborative system should enable users to seamlessly participate in the preference elicitation and decision-making process through natural and flexible interaction mechanisms. Simultaneously, it should incorporate transparent mechanisms for the system to communicate its suggestions.\\
%This collaborative system needs to allow for natural and flexible interaction mechanisms for the user to be seamlessly involved in the process of preference elicitation and decision making on one hand, and transparent mechanisms for the system to communicate system suggestions, on the other.
% Finally, previous research \cite{simon2004construction} investigated preference construction within the paradigm of multi-attribute decision theory (MAUT; see e.g., \cite{edwards1992multiattribute}; Hammond, Keeney, \& Raiffa, 1999). In fact, the majority of decision support systems are based on multi-attribute utility theory (MAUT) \cite{keeney1993decisions} and, therefore, represent preferences in form of utility functions [R]. 
Finally, preference construction within the paradigm of multi-attribute decision theory (MAUT~\cite{edwards1992multiattribute,keeney1993decisions, Hammond, Keeney, \& Raiffa, 1999}) represents preferences in the form of utility functions or embeds them as constraints [R].
% As a result, constraint satisfaction techniques have been used to automate the process of decision making in various scenarios, as it is aligned with how humans make decisions in complex scenarios and especially when trafe-offs are needed \cite{simon2004construction}. 
As a result, constraint satisfaction techniques have been used to automate the process of decision-making in complex scenarios where humans consider trade-offs in their decision-making~\cite{simon2004construction}. 
% \bs{This last guideline needs to be simplified to clarify the main point: Preference construction as constraint satisfaction is the right approach to take as this is how humans do it, and that's what we did.}

While optimization models such as Constraint Programming (CP)  are a natural fit for solving this complex reasoning problem and have been successfully applied in a range of multi-attribute decision problems, traditional optimization approaches require full knowledge of the model's specification - including a fully specified objective and all relevant constraints. This is at odds with how users approach complex and contextual decision-making tasks where they often do not know relevant preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most users. 
Finally, these optimization approaches must function as reasoning engines in dynamic and incremental settings. Here, users actively construct and adjust their preferences, while the system continuously learns and embeds their preferences and offers increasingly improved suggestions until a satisfactory one is achieved. 
% \bs{Shift to introducing our framework.}

% In this paper, we explore an innovative framework that integrates Large Language Models (LLMs) with optimization models. This combination leverages the versatility of LLMs as powerful multi-purpose tools, offering adaptable interactivity and advanced language understanding across various human-in-the-loop applications. \bs{A placeholder for now ...}
In this paper, we explore an innovative framework that supports an iterative preference elicitation that aligns with how humans develop or construct preferences in their decision-making and where elicited preferences are embedded into specific constraints that can be solved within an optimization setting.
We leverage (1) Large Language Models (LLMs) to facilitate natural and intuitive communication of preferences and suggestions as well as to reason about how preferences should be incorporated and translated into structured constraint functions and (2) CP techniques to reason over the space of outcomes and find optimal solutions given incorporated constraints. 
% \bs{Add(?): In this work we are exploring the design of an effective preference elicitation interface that is aligned with how humans preferences develop throughout the decision making process ...}
%\bs{Thinking of mentioning meeting scheduling as our scenario or use case for evaluating along with other aspects of the evaluation including the diary study and final user study.}
We evaluate this framework through the lens of meeting scheduling, a highly contextualized, personal, complex spatial-temporal decision-making process that requires users to reason over not only their existing meetings but also the complex temporal dynamics that govern their day. 
% We elaborate on different properties of meeting scheduling tasks in Section \ref{sec:motivating} that makes this problem very suitable to evaluate our proposed framework.
% \bs{End with a summary of main contributions and findings. Currently they are partially covered in Section 3.}
We introduce \system, a hybrid LLM and optimization approach that capitalizes on the benefits of both tools to build an interactive optimization system for meeting scheduling. 

Through a diary study, we find and characterize users' contextual scheduling preferences and quantitatively validate that our system is able to handle the majority of user preferences. 

Main contribution is testing the loop and the system is built to test the loop
\cl{Sentence or two on user study results.} We summarize our main contributions as follows:
\begin{itemize}
\item We designed and developed \system, a hybrid LLM and constraint programming system for interactive meeting scheduling.
\item To inform the design of the system, we ran a diary study (n=XXX) to find and characterize user's contextual scheduling preferences.
\item We created a new benchmark dataset for natural language for constraint programming and use it to quantitatively evaluate different components of \system. 
\item We ran a small-scale user study (n=XXX) to gauge the feasibility of the system and inform future design recommendations.
\end{itemize}



\begin{comment}
\bs{Transition to meeting scheduling as our use case and justifying the characteristics of meeting scheduling that makes it a suitable scenario to explore preference elicitation for}\\ 
While many wide-spread decision making and negotiation problems share these characteristics, we focus our work on meeting scheduling, as an example of a naturally distributed agreement problem, which is also known to be a tedious and time consuming daily activity for millions of information workers.
Meeting scheduling is a complex spatial-temporal decision-making process that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. For instance, ...
The user makes scheduling decisions considering diverse factors. Whether the user is initiating a new meeting or responding to a meeting request she chooses an action with multiple objectives in mind [Rs]. For instance, when trying to schedule a new meeting at a preferred time and location, the user may also want to minimize change to her existing meetings, and she takes a scheduling action that best compromises the overall objectives. These objectives could in turn comprise of multiple criteria such as: travel time, minimizing wait time, maximizing a contiguous meeting time, choosing a preferred meeting location, minimizing a variance from a preferred meeting time, maximizing the attendees who are desirable, or scheduling the calendar event as close as possible to a target date.


\bs{Placeholder for limitations of existing approaches}\\ 
Existing interfaces aiming at eliciting preferences from users range from systems that explicitly ask their users to fill in a long list of values for all the attributes of a certain item to systems that implicitly learn preferences from the user’s ratings or past behavior and comparison to other users of the system [R]. Both extremes are not likely to be successful if we want the user to stay engaged with the system and trust the system’s advice. First of all it is not sensible to ask a large number of elicitation questions that are cognitively demanding to the user. Using implicit techniques to get a preference model on the other hand bears the danger that the elicited model is not accurate [R]. This might lead to the problem that the users cannot comprehend the advice from the system.

\bs{Transition to design implications of past research that guided our design choices for this hybrid LLM-CP approach.}\\
Designing effective decision support systems (DSS) requires careful consideration of several key requirements.

(1) Interactivity: these systems must be interactive and actively engage the user in the user in the process of eliciting and revising their preferences, and adapt to their changing needs and goals.
% these systems must be interactive and actively engage the user in a dynamic and adaptive preference elicitation process.
The user interface should be clear, intuitive, and responsive, and allow the user to communicate their preferences easily and accurately.

%Secondly, these systems should seamlessly combine recommendations with preference elicitation, allowing users to refine their criteria and preferences as they explore options. This helps users make well-informed decisions.
(2) Interleaving: The DSS should not separate the phases of preference elicitation and recommendation generation, but rather interleave them in the same flow. This way, the user can learn from concrete examples, refine their criteria, and compare alternatives in an iterative and dynamic manner. The DSS should also provide critiquing mechanisms, such as explanations, feedback, and suggestions, to help the user evaluate and revise their preferences and decisions.

% Lastly, it's crucial to integrate the system into the task flow, as users may discover new preference criteria in specific situations. Adapting to factors like task complexity and time pressure is vital for providing valuable support. 
(3) Contextualization: these systems need to be contextualized and integrated into the task flow, as users may discover new preference criteria in specific situations.
% In summary, successful decision support systems should be interactive, integrate recommendations well, and be context-aware to support informed decision-making effectively.

\bs{Our focus and contributions.}\\
Large Language Models (LLMs) have emerged as a promising tool for helping accomplish a number of tasks such as generating code, writing, and visualizing data. However, they are well known to suffer from hallucinations and poor mathematical reasoning skills. This is particularly challenging in the context of meeting scheduling, which itself is a complex mathematical reasoning problem that has to both find times that satisfy scheduling requirements (i.e. constraint satisfaction) and reason over the relative importance of different constraints. Optimization models, such as Constraint Programming (CP), are a natural fit for solving the complex reasoning problems in scheduling and have been successfully applied in a number of large-scale industrial settings. However, traditional optimization approaches require full knowledge of the model's specification - including a fully specified objective and all relevant constraints. This is at odds with how users approach meeting scheduling - a highly contextual problem where users often do not know relevant constraints or preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most scheduling users.

In this paper we introduce \system, a hybrid LLM and optimization approach that capitalizes on the benefits of both tools to build an interactive optimization system for meeting scheduling. The system leverages LLMs to translate user chat history into structured scheduling constraints, represented by python functions, that can be used within a CP framework for generating improved meeting time suggestions. The framework benefits from the flexibility of LLMs to translate natural language into a structured form, while leveraging the power of optimization to do the reasoning over suggested times. Through a diary study, we find and characterize user's contextual scheduling preferences and constraints and quantitatively validate that our system is able to handle the majority of user preferences. \cl{Sentence or two on user study results.} We summarize our main contributions as follows:
\begin{itemize}
\item We designed and developed \system, a hybrid LLM and constraint programming system for interactive meeting scheduling.
\item To inform the design of the system, we ran a diary study (n=XXX) to find and characterize user's contextual scheduling preferences.
\item We created a new benchmark dataset for natural language for constraint programming and use it to quantitatively evaluate different components of \system. 
\item We ran a small-scale user study (n=XXX) to gauge the feasibility of the system and inform future design recommendations.
\end{itemize}
\end{comment}

 




==> deprecated/introduction-new-backup.tex <==
\section{Introduction}
% \bs{At a high level, this first draf of the Introduction needs to be shortened + it has more on the context setting than our actual contributions and what we are proposing. Some of that is covered in Section 3.}\\
%\bs{Continuing to work on the Inro but framing is getting there. Needs to be shorten at some point.}\\
% Knowing what a user likes and dislikes, i.e., their preferences, is important for intelligent systems in many domains. Users' preferences and constraints are particularly crucial for the success of systems that provide decision or negotiation support. 
Understanding what a user likes and dislikes, i.e., their preferences, is crucial for the success of intelligent systems that provide decision and negotiation support across many domains.
% Decision support systems, while sharing many similarities with Recommender Systems,  focus more on the decision process itself. This includes helping the user to discover and enter their preferences, understand the link between preferences and decision outcomes and analyzing the steps taken in the process.
Decision support systems target the decision process itself in helping the user discover and articulate their preferences, understanding the link between preferences and decision outcomes, and analyzing the steps taken in the process.
However, eliciting preference information from a user that informs such a decision process is challenging. This challenge manifests not only as the limitation of the algorithms for elicitating or representing preferences but also as the inherent difficulty of users knowing about or expressing their desired solutions. 

Prior psychology research~\cite{lichtenstein2006construction,Slovic1995construction} has shown that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions, attributing to the inherent limitations of individuals' memory, attention, and knowledge. 
In many situations, individuals do not really know what they prefer.
Rather, while a variety of preferences are carried in memory, the preferences are constructed as the situation arises~\cite{payne1992behavioral,payne1993adaptive} when (1) some decision elements may be unfamiliar to the individual; (2) the available choices may present a conflict among known preferences (i.e., trade-offs are needed); and (3) it is difficult to translate positive and negative feelings into a numerical response, even when the preferences are clear.
In these situations, the space of possible outcomes is too large to explicitly enumerate, and the solution must be synthesized via constrained optimization. 
These challenges are shared across widespread decision-making scenarios, such as meeting scheduling, purchasing, or resource allocation.

Preference elicitation tools and techniques \cite{goldsmith2008preference} (Section \ref{subsec:ElicitationTechniques}) are known to assist the human decision-maker in overcoming some of their inherent memory or knowledge limitations. However, the constructive nature of human preferences implies that the interaction between the system and a user can greatly influence the quality of the preference information [R] and the user's acceptance of the results provided by the system \cite{carenini2002constructed}.
Essentially, a preference elicitation interface needs to extract information from the user's mental representation of that preference and translate it into a representation the system can reason within an iterative, non-linear process.% Yet, this translation process entails an iterative loop and is not a linear, one-way process. 
% Preference modeling thus always involves three compo-nents: mental representation, elicitation and the system’s preference representation. 
\bs{Add(?): In this work we are exploring the design of an effective preference elicitation interface that is aligned with how humans preferences develop throughout the decision making process ...}
% In this paper, we focus on the design of an interactive preference elicitation interface which connects the two sides of this loop. 

% The main requirements of our design in simpler terms
% Interactivity --> human+system collaboration
% Contextualized
% Interleaving
% Transparency


The existing literature on adaptive decision making theory [R], preference construction [R] and decision making by constraint satisfaction [R] have provided a few guidelines for the design of effective decision support systems that actively support their users throughout the process of preference elicitation and decision making.\\ 
First of all, the preference construction process is highly influenced by the decision context and the way the preference elicitation is handled. Therefore, it's important for the elicitation mechanism to show decision context, that also allows people to see the consequences of their decisions. This can be further supported by providing specific examples that can be critiqued by the users to refine their preferences as well as immediate feedback that allows the users better understand the link between their stated preferences (constraints) and the suggestions provided by the system.\\
Second, as established in decades of HCI research, a major factor in designing effective and personalized decision support systems is the collaboration between the system and the user. Even the best underlying algorithms and reasoning frameworks do not give successful results if the user has problems interpreting information presented by the system and entering their preferences \cite{peintner2008preferences}. 
This collaborative system should enable users to seamlessly participate in the preference elicitation and decision-making process through natural and flexible interaction mechanisms. Simultaneously, it should incorporate transparent mechanisms for the system to communicate its suggestions.\\
%This collaborative system needs to allow for natural and flexible interaction mechanisms for the user to be seamlessly involved in the process of preference elicitation and decision making on one hand, and transparent mechanisms for the system to communicate system suggestions, on the other.
Finally, previous research \cite{simon2004construction} investigated preference construction within the paradigm of multi-attribute decision theory (MAUT; see e.g., \cite{edwards1992multiattribute}; Hammond, Keeney, \& Raiffa, 1999). In fact, the majority of decision support systems are based on multi-attribute utility theory (MAUT) \cite{keeney1993decisions} and, therefore, represent preferences in form of utility functions [R]. As a result, constraint satisfaction techniques have been used to automate the process of decision making in various scenarios, as it is aligned with how humans make decisions in complex scenarios and especially when trafe-offs are needed \cite{simon2004construction}. \bs{This last guideline needs to be simplified to clarify the main point: Preference construction as constraint satisfaction is the right approach to take as this is how humans do it, and that's what we did.}

While optimization models such as Constraint Programming (CP)  are a natural fit for solving the complex reasoning problems and have been successfully applied in a range of multi-attribute decision problems, traditional optimization approaches require full knowledge of the model's specification - including a fully specified objective and all relevant constraints. This is at odds with how users approach complex and contextual decision making tasks where they often do not know relevant constraints or preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most users. 
Finally, these optimization approaches must function as reasoning engines in dynamic and incremental settings. Here, users actively construct and adjust their constraints, while the system continuously learns their preferences. It then utilizes this information to offer increasingly improved recommendations until a satisfactory one is achieved. 
% Finally, these optimization approaches need to be employed as reasoning engines in highly interactive and flexible settings where users are actively constructing and revising their constraints on one end and the system interactively learning their preferences, and using them to suggest progressively better recommendations until a satisfactory one is found, on the other.

\bs{Shift to introducing our framework.}
% With the recent provision of Large Language Models and their application as multi-purpose tools that can provide highly flexible interactivity and language understanding in a range of human-in-the-loop application we are investigating a novel framework that combines LLMs with optimization models to facilitate interactive decision support. 
We are currently exploring an innovative framework that integrates Large Language Models (LLMs) with optimization models. This combination leverages the versatility of LLMs as powerful multi-purpose tools, offering adaptable interactivity and advanced language understanding across various human-in-the-loop applications. \bs{A placeholder for now ...}

%\bs{Thinking of mentioning meeting scheduling as our scenario or use case for evaluating along with other aspects of the evaluation including the diary study and final user study.}
We evaluate this framework through the lense of meeting scheduling, a highly contextualized and personal decision problem. 
Meeting scheduling is a complex spatial-temporal decision-making process that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. We elaborate on different properties of meeting scheduling tasks in Section \ref{sec:motivating} that makes this problem very suitable to evaluate our proposed framework.
\bs{End with a summary of main contributions and findings. Currently they are partially covered in Section 3.}



% Eliciting preference information from a user is challenging. On one hand, the user may not be fully aware of their preferences or be able to express it (at least via the elicitation mechanism offered) \cite{berry2007balancing}. On the other hand, even in cases where the user does know about their preferences and is able to express them, she may not be willing to input them to the system, especially if the elicitation process is burdensome. Moreover, the very process of elicitation itself is known to reshape — and at worst bias — the information provided; preferences can even be created by the elicitation process \cite{payne1993adaptive, viappiani2006evaluating}. 

% Psychology research has shown that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions \cite{Slovic1995construction} (for a comprehensive review, see \cite{lichtenstein2006construction}). 
% There is a body of literature that suggests people often do not have well-defined preferences. Instead they construct them during the elicitation process. Put differently, preferences are invented rather than found (Johnson, Steffel, \& Goldstein, 2005), more like the product of architecture than of archaeology (Gregory, Lichtenstein, \& Slovic, 1993; Payne, Bettman, \& Schkade, 1999). This implies that the interaction between the system and a user can greatly influence the quality of the preference information and the user’s acceptance of the results provided by the system. 

% Past research has also attributed these findings to the inherent limitations of individuals memory, attention and knowledge. Preference elicitation tools and techniques [Rs] are known to assist the human decision maker in overcoming these limitations. These computational aids can assist humans in identifying good quality solutions by interactively learning their preferences, which are unobserved, and using them to suggest progressively better recommendations until a satisfactory one is found.

% The central idea is that in many situations we do not really know what we prefer; rather, we must construct our preferences as the situation arises. While we do carry a variety of preferences in our memory, the need for preference construction arises when our known preferences are insufficient to solve the decision problem that we face. Past research has identified three main characteristics of situations where preferences need to be constructed through the course of an elicitation process: (1) some decision elements may be unfamiliar to the individual; (2) the choices available to us may present a conflict among our known preferences; and (3) in situations where we find it difficult to translate our positive and negative feelings into a numerical response, even when our preferences are clear.
% \bs{Also adding:} In these settings, the full set of outcomes is humongous and can not be explicitly enumerated, and the solution must be synthesized via constrained optimization. 




\begin{comment}
\bs{Transition to meeting scheduling as our use case and justifying the characteristics of meeting scheduling that makes it a suitable scenario to explore preference elicitation for}\\ 
While many wide-spread decision making and negotiation problems share these characteristics, we focus our work on meeting scheduling, as an example of a naturally distributed agreement problem, which is also known to be a tedious and time consuming daily activity for millions of information workers.
Meeting scheduling is a complex spatial-temporal decision-making process that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. For instance, ...
The user makes scheduling decisions considering diverse factors. Whether the user is initiating a new meeting or responding to a meeting request she chooses an action with multiple objectives in mind [Rs]. For instance, when trying to schedule a new meeting at a preferred time and location, the user may also want to minimize change to her existing meetings, and she takes a scheduling action that best compromises the overall objectives. These objectives could in turn comprise of multiple criteria such as: travel time, minimizing wait time, maximizing a contiguous meeting time, choosing a preferred meeting location, minimizing a variance from a preferred meeting time, maximizing the attendees who are desirable, or scheduling the calendar event as close as possible to a target date.


\bs{Placeholder for limitations of existing approaches}\\ 
Existing interfaces aiming at eliciting preferences from users range from systems that explicitly ask their users to fill in a long list of values for all the attributes of a certain item to systems that implicitly learn preferences from the user’s ratings or past behavior and comparison to other users of the system [R]. Both extremes are not likely to be successful if we want the user to stay engaged with the system and trust the system’s advice. First of all it is not sensible to ask a large number of elicitation questions that are cognitively demanding to the user. Using implicit techniques to get a preference model on the other hand bears the danger that the elicited model is not accurate [R]. This might lead to the problem that the users cannot comprehend the advice from the system.

\bs{Transition to design implications of past research that guided our design choices for this hybrid LLM-CP approach.}\\
Designing effective decision support systems (DSS) requires careful consideration of several key requirements.

(1) Interactivity: these systems must be interactive and actively engage the user in the user in the process of eliciting and revising their preferences, and adapt to their changing needs and goals.
% these systems must be interactive and actively engage the user in a dynamic and adaptive preference elicitation process.
The user interface should be clear, intuitive, and responsive, and allow the user to communicate their preferences easily and accurately.

%Secondly, these systems should seamlessly combine recommendations with preference elicitation, allowing users to refine their criteria and preferences as they explore options. This helps users make well-informed decisions.
(2) Interleaving: The DSS should not separate the phases of preference elicitation and recommendation generation, but rather interleave them in the same flow. This way, the user can learn from concrete examples, refine their criteria, and compare alternatives in an iterative and dynamic manner. The DSS should also provide critiquing mechanisms, such as explanations, feedback, and suggestions, to help the user evaluate and revise their preferences and decisions.

% Lastly, it's crucial to integrate the system into the task flow, as users may discover new preference criteria in specific situations. Adapting to factors like task complexity and time pressure is vital for providing valuable support. 
(3) Contextualization: these systems need to be contextualized and integrated into the task flow, as users may discover new preference criteria in specific situations.
% In summary, successful decision support systems should be interactive, integrate recommendations well, and be context-aware to support informed decision-making effectively.

\bs{Our focus and contributions.}\\
Large Language Models (LLMs) have emerged as a promising tool for helping accomplish a number of tasks such as generating code, writing, and visualizing data. However, they are well known to suffer from hallucinations and poor mathematical reasoning skills. This is particularly challenging in the context of meeting scheduling, which itself is a complex mathematical reasoning problem that has to both find times that satisfy scheduling requirements (i.e. constraint satisfaction) and reason over the relative importance of different constraints. Optimization models, such as Constraint Programming (CP), are a natural fit for solving the complex reasoning problems in scheduling and have been successfully applied in a number of large-scale industrial settings. However, traditional optimization approaches require full knowledge of the model's specification - including a fully specified objective and all relevant constraints. This is at odds with how users approach meeting scheduling - a highly contextual problem where users often do not know relevant constraints or preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most scheduling users.

In this paper we introduce \system, a hybrid LLM and optimization approach that capitalizes on the benefits of both tools to build an interactive optimization system for meeting scheduling. The system leverages LLMs to translate user chat history into structured scheduling constraints, represented by python functions, that can be used within a CP framework for generating improved meeting time suggestions. The framework benefits from the flexibility of LLMs to translate natural language into a structured form, while leveraging the power of optimization to do the reasoning over suggested times. Through a diary study, we find and characterize user's contextual scheduling preferences and constraints and quantitatively validate that our system is able to handle the majority of user preferences. \cl{Sentence or two on user study results.} We summarize our main contributions as follows:
\begin{itemize}
\item We designed and developed \system, a hybrid LLM and constraint programming system for interactive meeting scheduling.
\item To inform the design of the system, we ran a diary study (n=XXX) to find and characterize user's contextual scheduling preferences.
\item We created a new benchmark dataset for natural language for constraint programming and use it to quantitatively evaluate different components of \system. 
\item We ran a small-scale user study (n=XXX) to gauge the feasibility of the system and inform future design recommendations.
\end{itemize}
\end{comment}

 




==> deprecated/introduction.tex <==
\section{Introduction}


%Some of the text in this paragraph is from the CSCW background :)
Scheduling a meeting is tough! It is a complex spatial-temporal task that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. For instance, when trying to schedule a new meeting, the user may want to minimize change to her existing meetings, and she takes a scheduling action that best compromises the overall objectives, such as: minimizing travel time, maximizing a contiguous meeting time, choosing a preferred meeting location, etc. This has been further exacerbated by shifts towards remote work induced by COVID-19~\cite{teevan2022microsoft, yang2022effects}, blurring the boundary between work and personal life~\cite{allen2021boundary,hakkila2020practical}. It is therefore unsurprising, given the complex temporal dynamics governing people's workday, that scheduling is a complex personal behaviour. It is also an exceedingly contextual problem. Recent studies have shown that users often compromise on stated scheduling preferences for specific meetings.\footnote{\cl{Put this in reference to CSCW paper that showed stated preferences don't match exhibited behaviour but not sure how to reference.}} As a result, a calendar scheduling system that tries to predict the best scheduling actions needs to know user's preferences and priorities \cite{oh2005calendar} and the context to which it is being applied. However, existing calendaring tools present a rigid `one-size-fits-all` approach to generating suggested meeting times, giving users little recourse to customize the tool to their own complex scheduling preferences.

Large Language Models (LLMs) have emerged as a promising tool for helping accomplish a number of tasks such as generating code, writing, and visualizing data. However, they are well known to suffer from hallucinations and poor mathematical reasoning skills. This is particularly challenging in the context of meeting scheduling, which itself is a complex mathematical reasoning problem that has to both find times that satisfy scheduling requirements (i.e. constraint satisfaction) and reason over the relative importance of different constraints. Optimization models, such as Constraint Programming (CP), are a natural fit for solving the complex reasoning problems in scheduling and have been successfully applied in a number of large-scale industrial settings. However, traditional optimization approaches require full knowledge of the model's specification - including a fully specified objective and all relevant constraints. This is at odds with how users approach meeting scheduling - a highly contextual problem where users often do not know relevant constraints or preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most scheduling users.

%Introduce \system, hybrid LLM and optimization approach to generating new meeting times. Give a high level description of how system closes gap we discussed before. 

In this paper we introduce \system, a hybrid LLM and optimization approach that capitalizes on the benefits of both tools to build an interactive optimization system for meeting scheduling. The system leverages LLMs to translate user chat history into structured scheduling constraints, represented by python functions, that can be used within a CP framework for generating improved meeting time suggestions. The framework benefits from the flexibility of LLMs to translate natural language into a structured form, while leveraging the power of optimization to do the reasoning over suggested times. Through a diary study, we find and characterize user's contextual scheduling preferences and constraints and quantitatively validate that our system is able to handle the majority of user preferences. \cl{Sentence or two on user study results.} We summarize our main contributions as follows:
\begin{itemize}
\item We designed and developed \system, a hybrid LLM and constraint programming system for interactive meeting scheduling.
\item To inform the design of the system, we ran a diary study (n=XXX) to find and characterize user's contextual scheduling preferences.
\item We created a new benchmark dataset for natural language for constraint programming and use it to quantitatively evaluate different components of \system. 
\item We ran a small-scale user study (n=XXX) to gauge the feasibility of the system and inform future design recommendations.
\end{itemize}


==> deprecated/introduction_dec2023.tex <==
\section{Introduction}

Scheduling a meeting is tough! It is a complex spatiotemporal task that requires users to not only reason over their existing meetings, but also the complex temporal dynamics that govern their workday. For instance, when trying to schedule a new meeting, the user may want to minimize change to their existing meetings and takes a scheduling action that best compromises the overall objectives, such as: minimizing travel time, maximizing a contiguous meeting time, choosing a preferred meeting location, etc. This has been further exacerbated by shifts towards remote work induced by COVID-19~\cite{teevan2022microsoft, yang2022effects}, blurring the boundary between work and personal life~\cite{allen2021boundary,hakkila2020practical}. It is therefore unsurprising, given the complex temporal dynamics governing people's workday, that scheduling is a complex personal behaviour. It is also an exceedingly contextual problem. Recent results have shown that users often compromise on stated scheduling preferences for specific meetings \cite{baharcscw}. As a result, a calendar scheduling system that tries to predict the best scheduling actions needs to know user's preferences and priorities \cite{oh2005calendar} and the context to which it is being applied. 

However, understanding what a user likes and dislikes, i.e., their preferences, to inform when to schedule a meeting is challenging. Individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions which can be attributed to the inherent limitations of individuals' memory, attention, and knowledge ~\cite{lichtenstein2006construction,Slovic1995construction, payne1992behavioral, payne1993adaptive}. 
These challenges are shared across widespread decision-making scenarios, such as meeting scheduling, travel planning or purchasing a house. Preference elicitation tools and techniques \cite{goldsmith2008preference} are known to assist human decision-makers in overcoming some of their inherent memory or knowledge limitations, extracting information from the user's mental representation of that preference and translating it into a representation through which the system can reason. However, the constructive nature of human preferences implies that the interaction between the system and a user can greatly influence the quality of the preference information \cite{chen2009interaction, pommeranz2012designing, johnson2005making} and the user's acceptance of the results provided by the system \cite{carenini2002constructed, bettman1998constructive}. Prior work has shown that such preference elicitation systems need to be \textit{collaborative} to facilitate seamless information exchange between the user and the system ~\cite{peintner2008preferences}, \textit{contextualized} to the decision-making process \cite{payne1993adaptive, Slovic1995construction, pu2003user, carenini2002constructed}, and \textit{incremental} to account for evolving preferences \cite{pu2003user, pommeranz2012designing, ardissono2003framework}. Large Language Models (LLMs) provide a promising opportunity to support the naturalistic and contextual elicitation of user scheduling preferences via chat. Unlike prior systems that required all scheduling features and preferences to be known upfront \cite{brzozowski2006grouptime}, or require a user to manually specify all availability (e.g., doodle and when2meet), LLMs can allow users to specify in natural language a wider array of potential scheduling preferences (e.g., wanting a 10 minute break after meetings) that could be time consuming to input manually.


However, even once preferences are elicited, finding a solution that best meets them represents a challenging decision making task. Optimization models such as Constraint Programming (CP)  are a natural fit for solving complex reasoning problems arising in meeting scheduling and have been successfully applied in a range of multi-attribute decision problems. CP specifically aligns with multi-attribute decision theory \cite{edwards1992multiattribute,keeney1993decisions, hammond2015smart} where preferences are represented as utility functions or embedded as constraints, and constraint satisfaction techniques are leveraged to manage trade-offs ~\cite{simon2004construction}. However, traditional optimization approaches require full knowledge of the model's specification---including a fully specified objective and all relevant constraints. This is at odds with how users approach complex and contextual decision-making tasks where they often do not know relevant preferences unless presented with candidate solutions. Furthermore, customizing optimization models requires expertise in coding and optimization, an unrealistic barrier for most users. 
Finally, these optimization approaches must function as dynamic and incremental reasoning engines: users actively construct and adjust their preferences while the system continuously learns and embeds their preferences, offering increasingly improved suggestions until a satisfactory one is achieved. 
% \bs{Shift to introducing our framework.}

In this paper, we explore a novel framework that supports  iterative preference elicitation for meeting scheduling, aligning with how humans develop or construct preferences in their decision-making. Elicited scheduling preferences are embedded into specific constraints that can be solved within an optimization setting.
We leverage (1) Large Language Models (LLMs) to facilitate natural and intuitive communication of preferences and suggestions as well as to reason about how preferences should be incorporated and translated into structured constraint functions and (2) CP techniques to reason over the space of outcomes and find optimal solutions given incorporated constraints. 

We introduce \system, a hybrid LLM and CP approach that capitalizes on the benefits of both technologies to build an interactive decision support system for meeting scheduling. 
\system~ is designed to facilitate human-system collaboration that encompasses two key components: Preference Construction and Preference Incorporation. \textit{Preference Construction} is the process by which users of the system \textit{evaluate} candidate decisions (i.e., suggested meeting times) and \textit{express} new preferences and constraints that need to be integrated into the system. \textit{Preference Incorporation} is a mirror of the construction process from the system perspective and involves \textit{embedding} expressed user preferences in a form that can be used by the system to \textit{generate} new suggested decisions. We refer to the entire process of iteratively eliciting preferences via generating and critiquing suggestions as \textit{Preference Elicitation}. 
Because preference elicitation is an iterative process, \system~ unifies Preference Construction and Preference Incorporation into one dynamic loop where preferences are elicited in conjunction with refined suggestion generations. Figure \ref{fig:interaction_loop} outlines the key components of our interactive decision support system for meeting scheduling. 

We conducted three studies to better understand preference elicitation in the context of meeting scheduling.
First, we study how preferences are constructed via a diary study that collected naturalistic preferences in the moment of scheduling (n=64, Section \ref{sec:diary}). Our results highlight the diversity of user scheduling preferences, emphasizing the need for a system that can flexibly incorporate a wide range of preferences.
Informed by the results of the diary study, we then introduce \system~(Section \ref{sec:architecture}) and quantitatively evaluate the system's capabilities for preference incorporation (Section \ref{sec:quant_eval}).
Finally, we conduct a user study (n=10, Section \ref{sec:user_study}) with a prototype system to observe the iterative preference elicitation flow in situ and to inform future design improvements for interactive decision support systems.
Through our study, we confirm that participants' preferences are indeed constructed through the iterative preference elicitation process of evaluating dynamic time suggestions that incorporate their feedback.
We also identify that system explanations play a huge role in bridging the gap between understanding the system and expressing preferences, and contrasted suggestions can help give users a sense of agency.
Our work highlights the potential for a hybrid LLM and optimization approach for iterative preference elicitation and design considerations for building systems that support human-system collaborative decision-making processes.

%Loop description
 \begin{figure}[!t]
     \centering
      \includegraphics[width=\textwidth]{figures/interaction_loop.png}
         \vspace{-0.4cm}
           \caption{An overview of the interactive loop for conversational decision support. The loop is initiated via an initial time suggestion (or set of suggestions) by the system presented to the user (A). During \textit{Preference Construction} users evaluate a proposed suggestion (C) and either express a new preference (D) to improve the given suggestion, or accept the current suggestion. New preferences are integrated into the system during \textit{Preference Incorporation} which requires the system to both embed the stated preference into the system (W) and then use it to generate a new time suggestion (F). This process is iterated until a suitable time is found.
           }
\label{fig:interaction_loop}
\end{figure}


==> deprecated/related_work_commented.tex <==
\section{Related Work}
\label{sec:RW}
% Add a summary of what each of the subsections are and how it connects to our work.
% With respect to existing lit, it needs to be contextual and interactive. Current systems don't do that. LLM is good for but it's not for...Optimization is good for X but not for Y.
% Preference elicitation (what is it, how humans do it, how they are limited): Preference is constructed and not observed. People only become aware of it after interaction. In this paper, we design a system that helps people construct these preferences interactively.
% LLM supports this interaction, but it has limitations in reasoning. --> iterative process + LLM communication
% Optimization 
% ...

\subsection{Research on Human Preferences and Implications for Design}
\label{subsec:HumanPreferences}
\bs{This subsection is still WIP - Ignore for now}\\
%\bs{placeholder to add the research on how humans preferences devlope and what this means for system design?}
People's preferences have been the interest of researchers in many different fields including Psychology, (behavioral) decision making, consumer research, e-commerce, intelligent systems as well as negotiation and decision support. 
We focus on the key aspects of past research that are relevant for designing user interfaces for preference elicitation in (intelligent) decision support systems. 

Carenini and Poole \cite{carenini2002constructed} describe a conceptual shift for classical decision theory towards constructive preferences \cite{payne1993adaptive} and the implications for AI research. Opposing the prevailing economist view of rational and stable preferences, see e.g. \cite{doyle2004prospects}, psychology studies have confirmed that preferences are not stable but constructive. 
This is aligned with a substantial body of literature on judgment and decision-making has been devoted to the construction of preferences. It has been observed that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions \cite{Slovic1995construction}; (for a comprehensive review, see \cite{lichtenstein2006construction}). It has been suggested that preferences are invented rather than found \cite{johnson2005making}, more like the product of architecture than of archaeology (Gregory, Lichtenstein, \& Slovic, 1993; Payne, Bettman, \& Schkade, 1999). 

% Preference construction is an important element in a number of decision-making theories positing that the solution to decisional conflict lies in the reconstruction of the decision task (Janis \& Mann, 1977; Mills \& O’Neal, 1971; Montgomery, 1983; Montgomery \& Willen, 1999; Russo, Medvec, \& Meloy, 1996; Svenson, 1992, 1996). 

A shared premise of these theories is that people do not have well-defined preferences in most situations but rather construct them when necessary, i.e., in the decision-making context and in particular when decisional conflicts arise.
This line of research suggests that individuals can only feel confident in their decisions when one option clearly surpasses the others, which may involve adjusting initial preferences  \cite{simon2008transience}(Janis \& Mann, 1977; Mills \& O’Neal, 1971; Montgomery, 1983; Montgomery \& Willen, 1999; Russo, Medvec, \& Meloy, 1996; Svenson, 1992, 1996). This adaptive process enables individuals to reconstruct their preferences in response to new, crucial information. Therefore, for specific decisions, the gradual formation of preferences is a crucial and inseparable aspect of the decision-making process.

Due to the uncertainty nature of user goals and preferences, incremental elicitation of preferences has received much attention, where a user's preference model is improved over time as he or she interacts with the system. 
% Very little attention, however, has been paid to preference revision (Doyle and Thomason 1999). 
Other researchers both from behavioral decision theory and qualitative decision theory have also pointed out the advantage of eliciting user preferences incrementally \cite{pu2003user}. Continuous updates of the preference model and adaptations of the interface support the constructive nature of human preferences as they may evolve during the interaction with the system \cite{pommeranz2012designing, ardissono2003framework}. 


Preference construction was also investigated  within the paradigm of multi-attribute decision theory (MAUT; e.g., \cite{edwards1992multiattribute}; Hammond, Keeney, \& Raiffa, 1999)  \cite{simon2004construction}. The key insight is that the way individuals reconstruct their preferences in complex and decision making scenarios mimicks the constraint satisfaction process where preferences are represented in form of utility function.
To elaborate, this research has found while people processed the decision task, their preferences of attributes in the option that was  chosen increased whereas those for attributes of rejected options decreased. Similar effects have been found in negotiation settings reported by \cite{curhan2004dynamic}. This is in line with one  of the meta-goals named by Bettman and Luce \cite{bettman1998constructive}, i.e. trying to maximize the ease  of justifying a decision.
The studies by Simon, et al. \cite{simon2004construction} are part of a larger body of research on decision making by  constraint satisfaction that has found coherence shifts in a variety of tasks, including high-level reasoning  such as inductions, analogies, applications of rules to ambiguous situations, and social reasoning (Holyoak \&  Simon, 1999; Simon, Pham, Le, \& Holyoak, 2001), and various factual inferences (Simon, Snow, \& Read, 2004).

\begin{comment}
A substantial body of literature on judgment and decision-making has been devoted to the construction of preferences. It has been observed that individuals are often unsure of their preferences, hold inconsistent preferences, and change their preferences as they go about making decisions \cite{Slovic1995construction}; (for a comprehensive review, see \cite{lichtenstein2006construction}). It has been suggested that preferences are invented rather than found \cite{johnson2005making}, more like the product of architecture than of archaeology (Gregory, Lichtenstein, \& Slovic, 1993; Payne, Bettman, \& Schkade, 1999). Preference construction is an important element in a number of decision-making theories positing that the solution to decisional conflict lies in the reconstruction of the decision task (Janis \& Mann, 1977; Mills \& O’Neal, 1971; Montgomery, 1983; Montgomery \& Willen, 1999; Russo, Medvec, \& Meloy, 1996; Svenson, 1992, 1996). 

A shared premise of these theories is that confident and defensible decisions are possible when one of the decision alternatives become superior to its rivals, which requires that alternatives be ‘spread apart’ by altering the initial preferences of the decision’s attributes \cite{simon2008transience}. Thus, for certain decisions, the construction of preferences can be considered an integral and essential part of the decision-making process. 

Carenini and Poole \cite{carenini2002constructed} describe a conceptual shift for classical decision theory towards constructive preferences \cite{payne1993adaptive} and the implications for AI research. Opposing the prevailing economist view of rational and stable preferences, see e.g. \cite{doyle2004prospects}, psychology studies have confirmed that preferences are not stable but constructive. This means that people do not have well-defined preferences in most situations but rather construct them when necessary, i.e., in the decision making context. This allows people to re-construct their preferences whenever they get new information that is important for the decision. There are different views on how people construct their preferences.


\bs{Preference construction as constraint satisfaction}\\
Previous research \cite{simon2004construction} investigated preference construction within the paradigm of multi-attribute decision theory (MAUT; e.g., Edwards \& Newman, 1982; Hammond, Keeney, \& Raiffa, 1999).
They found while people processed the decision task, their preferences of attributes in the option that was  chosen increased whereas those for attributes of rejected options decreased. Similar effects have been found in negotiation settings reported by \cite{curhan2004dynamic}. This is in line with one  of the meta-goals named by Bettman and Luce \cite{bettman1998constructive}, i.e. trying to maximize the ease  of justifying a decision.

 The studies by Simon, et al. \cite{simon2004construction} are part of a larger body of research on decision making by
 constraint satisfaction that has found coherence shifts in a variety of tasks, including high-level reasoning
 such as inductions, analogies, applications of rules to ambiguous situations, and social reasoning (Holyoak \&
 Simon, 1999; Simon, Pham, Le, \& Holyoak, 2001), and various factual inferences (Simon, Snow, \& Read, 2004).
\end{comment}

%----- transitioning to the design implications of the research highlited in the first half of this subsection --
In order to build a system and in particular the interface of the system that is usable and supports the user in creating and entering his or her preferences system designers need to consider how human preferences develop.


Two main areas of relevant literature highlights the key requirements for designing effective decision support systems:
\bs{from the review of decades of Psychology and cognitive science litetature related to human preferences, the list under (2) seem to greatly provide implications for design.}


\textbf{(1) Human-System Interaction and Collaboration.}\\
% ChatGPT: Decades of research in Human-Computer Interaction (HCI) and user-centered design have underscored the critical importance of interactivity and collaboration in effective decision support systems. These systems are most successful when they actively engage users in the decision-making process, transforming it into a collaborative endeavor between human and machine. An interactive interface not only enables users to provide their preferences but also facilitates a dynamic exchange of information and ideas between the user and the system. This collaborative approach ensures that the decision-making process benefits from both human intuition and system-generated insights. By placing the user at the center of the decision-making loop and emphasizing a collaborative dynamic, these systems tap into the complementary strengths of both human cognition and computational capabilities, leading to more informed and robust decision outcomes. This foundational principle has significantly advanced the development of decision support systems, emphasizing the need for active user engagement and collaboration as pivotal components in their design and functionality.
Decades of research in Human-Computer Interaction (HCI) and user-centered design have underscored the critical importance of interactivity and collaboration in effective decision support systems. We highlight 3 main criteria for the interaction between the user and the system to enable collaborative deicision support based on this literature:
\begin{itemize}
    \item Interactivity and Natural Interaction (user to system direction): 
Users should play an active role in the preference elicitation process. The system's UI should offer easy-to-use mechanisms for users to communicate, revise, and provide feedback on their preferences and constraints, as well as critique system suggestions. This interaction should feel flexible, natural, and without unnecessary complexity.
    \item Iterative / Incremental Recommendation + Transparency (system to user direction)
    
\end{itemize}
\textbf{(2) Support for human process of constructing preferences.}
\begin{itemize}
    \item Preferences are constructed, not simply revealed (observed);
    \item Preference construction process is highly influenced by the \textit{decision context} and the way the preference elicitation is handled. In particular \cite{pu2003user}, the elicitation mechanism needs to show deicison context and allow people to see consequences of their decisions. This can be further supported by providing concrete examples that can be critiqued by the user to refine their preferences. Additionally, the system needs to provide immediate feedback, which would unlock the information flow from the system to the user and help the user understand the link between their stated preferences and constraints and proposed solutions.
    \item The preference elicitation process needs to be done incrementally and not in a single turn.
% Other researchers both from behavioral decision theory and qualitative decision theory have also pointed out the advantage of eliciting user preferences incrementally. 
    \item Preference construction mimicks the process of constraint satisfaction where preferences are represented in form of a utility function.
\end{itemize}


\subsection{Existing Preference Elicitation Techniques}
\label{subsec:ElicitationTechniques}
%\bs{The goal is not to review all existing techniques. The scope is pretty broad and includes both the RecSys literature and a more closely relevant area of Decision Support Systems. I'm aiming to provide references that provide extensive reviews of existing techniques for an interested reader and focus the section on a few approaches that are more relevant to our work + highlight some of the existing gaps of these techniques.}\\
%Preference elicitation (Goldsmith and Junker 2009) is a well-studied problem in artificial intelligence, recommender systems, and human-computer interaction. Various techniques and approaches have been proposed to infer user preferences from different types of feedback, such as rankings, corrections, critiques, ratings, from queries or from past behavior. \bs{TODO: add Refs for each.}

%Methods for acquiring user preferences vary in their degree of user involvement, depending on the system's nature. 
%Implicit methods involve the user in a less ``\textit{active}'' manner during the elicitation task compared to explicit methods.
%One example of implicit methods can be preference learning based on user behaviour (e.g., items the user looked at or bought or the traces of users interactions with an application). Users may still be aware of the workings of implicit methods and expect an interpretation of their actions. Most of these approaches are following Revealed Preference Theory (Samuelson, 1938) , which assumes that knowledge relating to user preferencse can be acquired by (passively) observing the user’s actions over time. \bs{elaborate on limitations of these appraoches.}

%Explicit approaches, on the other hand, involve obtaining specific preference input, like ratings. 
%The level of user involvement often requires balancing user effort with the richness of information required by learning algorithms driving personalized experiences \cite{schnabel2020doesn}.
%While on the lower-end of the information richness spectrum are systems that support simple user feedback such as ratings, on the upper end of the spectrum are systems such as chat bots that allow people to have conversations about their preferences. \bs{TODO: needs some references.}

Preference elicitation \cite{goldsmith2008preference} is a well-explored topic in artificial intelligence, recommender systems, and human-computer interaction.
Numerous techniques exist for inferring user preferences from various forms of feedback, including rankings, corrections, critiques, ratings, queries, and past behavior.
\textit{Implicit} methods, such as preference learning from user behavior, involve less active user participation during the elicitation process and align with Revealed Preference Theory~\citep{richter1966revealed}.
In contrast, \textit{explicit} approaches, like collecting ratings, require more direct user involvement.
The level of user engagement must be balanced with the depth of information needed for personalized experiences~\citep{schnabel2020doesn}.
This information can range from simple user feedback like ratings to more complex interactions, as seen in systems like chatbots facilitating conversations about preferences.


%A full review of the methods typically used in recommender systems together with examples representing typical systems in the area is outside the scope of this paper. For more exhaustive reviews in the area see (Chen and Pu 2004; Peintner et al. 2008). 
%We, however, highlight two techniques, enabled by the conversational models of recommender systems, that are more closely aligned with the constructive view of preferences and our present work.
%One of the first attempts to enable more conversational recommender systems comes from Carenini et al.(2003). They extended the traditional collaborative filtering techniques to a more conversational model which allowed the users and the system to ``\textit{work together}'' (collaborate) to improve the system's recommendations and the user experience. Since then, The interest in Conversational Recommender Systems has significantly increased in the past few years (See \cite{jannach2021survey} for a recent review of these systems). This development is mainly due to the significant progress in the area of natural language processing and the emergence of conversational agents. Two methods, derived from this conversational model, are `\textit{Example Similarity and Tweaking}' and `\textit{Example-Critiquing Interaction}'. Our work aligns with certain aspects of these techniques.

%Similarity and tweaking techniques involve two main steps. In the ﬁrst step the user selects an item from the system’s catalogue and requests similar items. The system then retrieves a large number of alternative items from its database, sorts them according to similarity to the chosen item and returns a small number of alternatives with highest similarity to the user. In case the system offers tweaking the process is essentially the same with the only difference that the user gives a tweak in the ﬁrst step, e.g., ``\textit{show me similar, but cheaper items}''. The system only returns items to the user that satisfy the tweak, that are cheaper in this case.
%\bs{How is our work similar to this technique? In our setting the user initiates the process by specifying certain attributes of the desired solution, e.g. the list of attendees and a duration for the meeting and receives initial time recommendations. The user can then ask for new recommendations by specifying attributes that are preferred and the ones that need to change.}

%A similar technique is example-critiquing or the candidate/critique model (Pu and Chen 2008). In example-critiquing users are presented with a set of candidates they can critique. Candidates have to motivate users to state their preferences and the most preferred solution needs to be among the displayed candidates (Faltingset al. 2004). 
%Several strategies have been proposed to select candidates, e.g., using extreme examples (Linden et al. 1997), diverse examples (Smyth and Mcginty 2003) or so called Pareto-strategies (Viappiani et al. 2005). In an iterative process the system learns the users' preferences from their critiques and updates the user models. Critiques can be system-suggested or user-initiated. \bs{Our system follows a similar iterative approach to learn users preferences and update time recommendations accordingly. It also provides mechanisms for the users to critique the time recommendations in the chat, e.g. by stating `\textit{let's avoid Fridays}' or `\textit{I don't want to meet during lunch time}'.}

We emphasize two conversational techniques closely related to our work.
%
The first technique, inspired by conversational recommender systems, encourages users and the system to collaborate in improving recommendations.
This approach has gained popularity due to advances in natural language processing and conversational agents.
Our work shares similarities with the \textit{Similarity and Tweaking} method, where users initiate recommendations by specifying attributes, just as our users specify meeting criteria~\citep{carenini2003towards,jannach2021survey}.
%
Another relevant technique is \textit{Example-Critiquing Interaction}~\citep{chen2012critiquing}, where users critique a set of candidates to express their preferences.
Our system follows a similar iterative approach to learn user preferences and offers mechanisms for users to critique time recommendations within the chat interface, such as specifying preferences like avoiding certain days or times.
%
For more exhaustive reviews in the area see~\citep{chen2004survey,peintner2008preferences}.

%DSS
%Our work is closely connected to another research area that specifically examines techniques for eliciting preferences within Decision Support Systems (DSS).
%Decision support systems are interactive systems that support users in taking decisions by eliciting preferences and offering analytical tools to scrutinize decisions. Unlike recommender systems that focus on finding the best outcome in a huge set of possible outcomes, decision support systems focus much more on the process of taking a decision and the role of preferences influencing that process.
%The majority of decision support systems are based on multi-attribute utility theory (MAUT) (Keeney and Raiffa 1993) and, therefore, represent preferences in form of utility functions. \bs{connection to our choice of constraint programming tools}.

%In order to construct utility functions the system needs to elicit values and weights for the given attributes of an item. 
%The two most popular preference elicitation techniques are absolute measurement and pairwise comparison (active elicitation) (Aloysius et al. 2006).  

%These approaches, however, may result in a potential mismatch between the user’s mental model of their preferences and the system's preference representation. This is mainly due to the discrepancy between the rational, quantitative models used in systems and the constructive, qualitative mental models of people. 
%First, rational models assume that people have stable and coherent preferences that are always known to them.
%This is not aligned with the research on the constructive view of preferences as reviewed in Section \ref{subsec:HumanPreferences}.
%In addition, it is difﬁcult for people to express their preferences in numerical attribute weights and values as needed by automated systems, particularly if they are not experts in the domain. Whereas people might easily state that they prefer, e.g., more holidays to less holidays specifying this relation in concrete numbers, such as ``\textit{I like 30 holidays 2.5 times as much as 28 holidays}'' is not intuitive. \bs{@Connor: we do not require users to specify weights for their preferences in our approach, rather we rank them by the recency of the order they are specified? Could you write a sentence on how we handle this?}

Our work is closely tied to another research area that focuses on preference elicitation in Decision Support Systems (DSS).
DSS are interactive tools designed to assist users in making decisions by gathering preferences and providing analytical tools to analyze these decisions.
%Unlike recommender systems, which aim to find the best outcome from a large set of possibilities, DSS emphasize the decision-making process and the influence of preferences on that process.
%
Most DSS rely on multi-attribute utility theory~\citep{keeney1993decisions} to represent preferences as utility functions.
This is relevant to our choice of constraint programming tools.
%
To construct these utility functions, the system must elicit values and weights for the attributes of an item.
The two most common preference elicitation techniques are absolute measurement and pairwise comparison (active elicitation)~\citep{aloysius2006user}.
%
However, these approaches can lead to a potential misalignment between the user's mental model of their preferences and the system's preference representation.
This discrepancy arises from the difference between the rational, quantitative models used by the systems and the more qualitative, constructive mental models of individuals.
Rational models assume that people have stable and consistent preferences that are always known to them, which contradicts the research on the constructive view of preferences discussed in Section \ref{subsec:HumanPreferences}.
%
Additionally, it can be challenging for individuals to express their preferences in the numerical attribute weights and values required by automated systems, especially if they are not experts in the domain.
While people might easily state a preference for more holidays over fewer holidays, specifying this preference in concrete numerical terms, such as ``I like 30 holidays 2.5 times as much as 28 holidays,'' is not intuitive.

%\bs{End this section with: Support of human preference construction in current methods. Revise the following and shortern.}\\

%In order to build a system and in particular the interface of the system that is usable and supports the user in creating and entering their preferences system designers need to consider how human preferences develop and support users in constructing their preferences accordingly.
%But in how far do the methods presented above actually take these aspects into consideration?

%Generally, the implicit methods do not actively involve users in constructing their preferences. Collaborative ﬁltering methods base their choices on the assumptions that similar people like similar things. However, there is always the danger that the system creates an erroneous user model and the user gets confused about seemingly unrelated recommendations. 

%Explicit methods focus more on the user. Conversational methods allow the users to construct and reﬂect upon preferences. Example critiquing has been explicitly developed based on the constructive view of human preferences. This is reﬂected in the attempts of improving the algorithms to pick examples that will help the users to uncover hidden preferences. Whereas tweaking and example-critiquing are widely used for recommenders, many decision support systems use active elicitation methods based on utility models. This requires users to enter values and weights in form of numbers. Other active elicitation methods like pairwise comparison do not require numbers but still assume that a user is able to compute which of the given options is better. With unknown items this is a difﬁcult task.

To create a user-friendly system, designers must consider how human preferences develop and guide users accordingly.
However, it is important to assess whether the methods mentioned earlier address these considerations.
%
Implicit methods do not actively involve users in shaping preferences.
Collaborative filtering relies on the assumption that similar people have similar preferences, which can lead to inaccurate user models and confusing recommendations.
%
Explicit methods are more user-centric.
Conversational methods let users construct and reflect on preferences, while example critiquing aligns with the constructive view of preferences by improving algorithms to help users uncover hidden preferences.
In contrast, many DSS use active elicitation methods based on utility models, requiring numerical input.
Pairwise comparison, another active method, assumes users can determine preference without numbers, but this can be challenging with unknown items.

\js{Add more references}



\begin{comment}
\subsection{Time Suggestion Tools}
\begin{itemize}
    \item Highlight existing work on time suggestions (i.e. Calendar dot help, RHCal, etc.)
    \item Thinking of leveraging Bahar's Literature Review on scheduling system to frame this.
    \item Contrast that many existing systems aren't interactive/grounded in the context of the meeting scheduling instance.
    \item For comparison to Calendar dot help might be worth contrasting level of automation/speed/distributed nature (i.e. we don't deal with the coordination problem, but are able to quickly automate convergence to a time from the organizer's perspective)
\end{itemize}
\end{comment}

\subsection{User Scheduling Preferences}
\bs{I'm thinking we should upload the CSCW paper on Arxiv to be able to cite it here and even refer to it for a review of past literature.}
Given the intricacies of people's workday schedules, scheduling becomes a complex personal behavior.
Whether a user is arranging a new meeting or responding to a request, they consider multiple objectives, such as minimizing disruptions, travel time, and preferred locations \cite{berry2007balancing,oh2005calendar}.
Therefore, an effective calendar scheduling system must understand user preferences \cite{oh2005calendar}.
%
Preference learning is crucial in various applications like decision support systems, recommender systems, and personalized devices~\citep{chajewska2000making, heskes2005incremental}.
%
Prior research has explored incorporating personal preferences into calendar scheduling systems \cite{dent1992personal,mitchell1994experience,sen1997satisfying,chajewska2000making,tullio2002augmenting,oh2005calendar,gervasio2005active,brzozowski2006grouptime,krzywicki2010adaptive,kim2018learning}.
For instance, Calendar Apprentice (CAP) by \citet{mitchell1994experience} uses decision trees to predict scheduling attributes. PLIANT \cite{gervasio2005active} adopts active learning.
%
However, understanding user preferences in scheduling systems faces challenges in preference elicitation. Users may not be fully aware of preferences or may find the process burdensome. Two primary approaches are used for preference elicitation: the example-driven approach (1) derives schedule rankings by presenting users with specific examples, as seen in GroupTime \cite{brzozowski2006grouptime}. Well-chosen examples can stimulate preferences \cite{viappiani2006evaluating}.
The model-driven approach (2) requires users to input preference model parameters directly, as in \citet{haynes1997automated}. While it shortens the elicitation period, users must understand the model.
\js{Which one is ours? Or none of them?}
%
Some systems, like PTIME \cite{berry2007balancing}, take a user-centered approach, capturing criteria through structured interviews and using an interactive interface. However, gaps in preference categories remain to be addressed.

\js{Relate this back to our work}


% Potentially a section on: Constraint/preference elicitation - Constraint/preference as a construct

\subsection{Large Language Models and Optimization}
%Alt title: Human-Centered Optimization, Collaborative Optimization...
% LLM is a great tool but lacks math reasoning ability. Here are approaches to augment reasoning.

%\cl{Stealing some of my wordering from the old introduction. Leaving this here as a reminder to reword if we end keeping parts of it.}

Large Language Models (LLMs) have emerged as a promising tool for helping accomplish a number of tasks such as generating code \cite{chen2021evaluating}, writing \cite{yuan2022wordcraft}, and visualizing data \cite{dibia2023lida}. However, they are well known to suffer from hallucinations, seemingly plausible text predictions that are in fact non-factual \cite{welleck2019neural}, and poor mathematical reasoning ability \cite{qian2022limitations}. Recent work have aimed to address these shortcomings by helping LLMs decompose complex tasks into simpler steps (e.g., \cite{wei2022chain, yao2022react,yao2023tree}) and augmenting them with external tools (e.g., \cite{schick2023toolformer, thoppilan2022lamda, nakano2021webgpt}) such as a code interpreter (see \citet{mialon2023augmented} for a survey of other related approaches). Our work builds upon this line of work by decomposing the complex problem of suggesting meeting times into structured sub-components (detailed in Section \ref{sec:architecture}). We also employ an optimization solver as an external tool to perform complex reasoning over meeting times. This is in contrast to other existing working on collaborative decision making between LLMs and humans such as \citet{lin2023decision} which requires the LLM to generate the solutions.

% Optimization bad at ambiguity
Mathematical optimization is a natural tool for tackling challenging mathematical reasoning problems, and have been successfully applied in a number of industrial applications such as supply chain management, scheduling, and inventory control \cite{bertsimas1997introduction}. In this paper we focus on (Weighted) Constraint Programming (see \citet{rossi1999constraint} for a survey of related work), a modelling paradigm where the optimization problem is defined by a set of arbitrary constraints that may have different weights. The goal is to find a solution that has the optimal score, defined by the total weight of all constraints it satisfies. However, traditionally constraint programming require a full specification of the underlying optimization model including all relevant constraints and weights with precise numerical coefficeints. This presents stark challenges for preference elicitation, where user's underlying constraints and preferences are often unknown and expressed in the context of proposed solutions. To help alleviate these shortcomings, there has been recent work on solving and formulating constraint programming problems with incomplete information where certian data and preferences need to be elicited \cite{tabakhi2021preference, tabakhi2022incomplete, tabakhi2017preference, xiao2020embedding, tabakhi2017preference2}. However, existing approaches focus on algorithmic elements of what information to elicit as opposed to the mechanism by which to elicit it. This is an important distinction in more general settings such as meeting scheduling, where non-expert users are unlikely to have the modelling expertise to understand and formulate constraints they want added to a model.

% NLP 4 Opt
Natural language processing techniques are a promising tool to help alleviate the technical barriers for non-expert users to interact with optimization models. Recent work has leveraged LLMs as a tool for users to ask counter-factual questions about models in applications such as supply chain management \cite{li2023large}, and identifying infeasible subsystems within an optimization model \cite{chen2023diagnosing}. However, these existing chat-based systems focus on facilitating understanding of an existing model, as opposed to the much more difficult task of constructing a new model. Motivated by this high technical barrier to formulating optimization problems, there has been a line of recent work focused on using tools from natural language processing to construct optimization models. \citet{ramamonjison2022augmenting} first introduced the problem of mapping natural language text descriptions to a formal optimization model. This was also the focus of the recent NL4Opt competition at NeurIPs \cite{ramamonjison2023nl4opt} which inspired related work focused on named entity recognition and semantic parsing for textual descriptions of optimization models \cite{ning2023novel, tsouros2023holy, dakle2023ner4opt, prasath2023synthesis}. This line of work focuses primarily on the static setting, where a single paragraph of text is translated into an optimization model. In contrast, we study an interactive model where we elicit natural language user preferences within the flow of constructing the optimization model. Our approach also focuses on translating natural language into python constraints within a constraint programming framework, as opposed to a more traditional named entity recognition appraoch which has been geared priarily to linear and integer programming. Our approach also focuses on a simpler underlying optimization model that eschews the need for formal optimization solvers.



%More of why are we talking about these things.

==> rebuttal_probe.tex <==
We briefly mentioned in our User Study section that ``we evalute the \system~system not as a finished product but as a probe~\cite{boehner2007hci}.'' 
The concept of using a ``probe'' as a provocational or an inspirational instrument to ``find out about the unknown—returning with useful or interesting data~\cite{hutchinson2003technology}'' has been well-established in the HCI literature for many decades~\cite{gaver1999design,graham2008probes,boehner2007hci,hutchinson2003technology}. However, our submitted paper failed to provide sufficient background describing this as a methodological approach. ``Technology as a probe'' is a method of research in HCI aimed at promoting participant engagement and insights during design. 

The dominant culture that values usability evaluations with controlled experiments or baseline systems as well as the quantitative evaluations has been a point of contention and criticism in the HCI academic community~\cite{greenberg2008usability} and a topic worth revisiting for examining this paper's contribution.
Rather than evaluating the usability or effectiveness of a certain technology to get the right design, we use technology probes to get the design right with a focus on inspiring users and researchers and identifying potential areas of improvement and considerations to arrive at the right design without eliminating ideas too early~\cite{greenberg2008usability}. 
Probes are meant to inspire design ideas rather than provide definitive answers to a single question~\cite{boehner2012probes}.

Given this methodological context, our user study was not a usability study where task success/failure rates could be measured or typical statistical comparisons could be made because we did not follow a protocol required for scientifically measuring task success rates. While we did capture such data, the study protocol was intentionally open-ended with active and ongoing conversation between users and researchers. This study design inherently introduces too many confounding variables to quantitatively compare tasks or users. Instead, it is important to highlight that our tasks were used as an elicitation tool for user reactions that were constantly inquired about. 

To fill this gap in expressing our intentions, we make the following revisions in our paper:
\begin{enumerate}
    \item We bring the necessary background on ``technology probe'' in our User Study section. We describe the HCI field's current understanding and usage of this method, and we outline how such understanding informs our analysis. 
    \item We consistently use of the term ``technology probe'' throughout the paper. We avoid the use of the term ``prototype'' that may come with an assumption that it is ready for usability testing.
    \item We make it clear that our study was not designed for traditional usability testing and for capturing quantitivate task success rates. We explicitly mention our elicitation focused methodology and discuss the limitations of such methodology.
\end{enumerate}

==> sections/motivating_example.tex <==
\section{Motivating Example: Meeting Scheduling}
\label{sec:motivating}

%\bs{@Connor: Really like this section! It was a right call to separate the scenario as a separate section. You've got most of it there already, but what I had in mind was to take some of the content on charactersitcs of meeting scheduling from the literature review doc here. In paricular: (1) Meeting scheduling is a routine, tedious, and time-consuming daily activity, which requires coordination and cooperation among all attendees. (something that highlights the commonality / scale of this task among information workers and hence the magnitude of the impact we could have if we effectively support this process) (2)  Meeting scheduling a well-known naturally distributed agreement problem and the main challenge is how to find agreed time among various constraints, such as participant’s schedules, preferences, or priorities. (3) [Property 1: incremental and continuous.] Research shows it is incremental and continuous. As opposed to reaching for a set of definite final goal states, scheduling is done in more or less a greedy fashion [11]. When faced with a meeting scheduling decision at a given point in time, the user typically chooses the option that looks best in this context. (4) [Property 2: complex personal behavior]  }
\bs{For a truly motivating example section, some concrete examples can go a long way (time permitting). See in-app comment.}\\
We study a novel framework for interactive decision support systems through the lens of meeting scheduling, a routine, tedious, and time-consuming daily activity faced by a multitude of information workers. At its core, scheduling a meeting is a complex spatial-temporal task that requires reasoning over participant's schedules, preferences, or priorities. Previous work has shown that scheduling is a complex personal behavior that is highly contextual, and finding a suitable meeting time may require reasoning over conflicting preferences and constraints \cite{baharcscw}. It is also an incremental and continuous process that requires iteratively refining candidate solutions in a more or less greedy fashion \cite{brzozowski2006grouptime}. Interactive decision support tools are a natural fit for scheduling as they can provide contextualized and interactive support for the complex reasoning that is necessary to complete the task. 

The goal of such a system is to work collaboratively with a user to help generate suggested meeting times. This human-system collaboration encompasses two key components: Preference Construction, and Preference Incorporation. \textit{Preference Construction} is the process by which users of the system \textit{evaluate} candidate decisions, in the context of meeting scheduling these are suggested meeting times, and \textit{express} new preferences and constraints that need to be integrated into the system. \textit{Preference Incorporation} is a mirror of the construction process from the system perspective and requires \textit{embedding} expressed user preferences in a form that can be used by the system to \textit{generate} new suggested decisions. We refer to the entire process of iteratively eliciting preferences via generating and critiquing suggestions as \textit{Preference Elicitation}. It is important to note that this is an interative process, and a main contribution of our work is to unify the two components into one dynamic loop where preferences are elicited in conjunction with the refined generation of suggestions. Figure \ref{fig:interaction_loop} outlines the key components of our interactive decision support system for meeting scheduling. 

%We decompose the problem into two primary components: Preference Construction, and Preference Incorporation. 
%Preference elicitation is the broader task of eliciting user preferences in response to decision suggestions, specifically suggested meeting times. It encompases three key phases: (A) Evaluation of suggested times, (B) Internal construction of a new preference in response to the time, and (C) the externalizing of that preference the system. Once a new preference has been articualted, the goal of the second component \textit{Preference Incorporation} is to integrate the preference to present a refined suggestion. 

The remainder of the paper endeavors to better understand preference construction in the context of meeting scheduling, and uses it inform the design of a novel system for preference incorporation. We study Preference Construction in the context of meeting scheduling via a diary study outlined in Section \ref{sec:diary}. Informed by the results of the diary study, we introduce a hybrid LLM and constraint programming framework for preference incorporation in Section \ref{sec:architecture}. The system capitalizes on the flexibility of large language models to translate natural language into structured forms to perform preference embedding, and leverages the reasoning ability of constraint programming to generate improved time suggestions based on the embedded preferences. To evaluate the proposed interactive decision support system we present a quantitative analysis of the preference incorporation system in Section \ref{sec:quant_eval} and a qualitative evaluation of the broader preference elicitation framework via a user study in Section \ref{sec:user_study}.
%Loop description
 \begin{figure}[!t]
     \centering
      \includegraphics[width=\textwidth]{figures/interaction_loop.png}
         \vspace{-0.4cm}
           \caption{An overview of the interactive loop for conversational decision support. The loop is initiated via an initial time suggestion (or set of suggestions) by the system presented to the user (A). During \textit{Preference Construction} users evaluate a proposed suggestion (C) and either express a new preference (D) to improve the given suggestion, or accept the current suggestion. New preferences are integrated into the system during \textit{Preference Incorporation} which requires the system to both embed the stated preference into the system (W) and then use it to generate a new time suggestion (F). This process is iterated until a suitable time is found.
           }
\label{fig:interaction_loop}
\end{figure}

